Scaling up self-supervised learning for improved surgical foundation models

Foundation models have revolutionized computer vision by achieving vastly superior performance across diverse tasks through large-scale pretraining on extensive datasets. However, their application in surgical computer vision has been limited. This study addresses this gap by introducing SurgeNetXL, a novel surgical foundation model that sets a new benchmark in surgical computer vision. Trained on the largest reported surgical dataset to date, comprising over 4.7 million video frames, SurgeNetXL achieves consistent top-tier performance across six datasets spanning four surgical procedures and three tasks, including semantic segmentation, phase recognition, and critical view of safety (CVS) classification. Compared with the best-performing surgical foundation models, SurgeNetXL shows mean improvements of 2.4, 9.0, and 12.6 percent for semantic segmentation, phase recognition, and CVS classification, respectively. Additionally, SurgeNetXL outperforms the best-performing ImageNet-based variants by 14.4, 4.0, and 1.6 percent in the respective tasks. In addition to advancing model performance, this study provides key insights into scaling pretraining datasets, extending training durations, and optimizing model architectures specifically for surgical computer vision. These findings pave the way for improved generalizability and robustness in data-scarce scenarios, offering a comprehensive framework for future research in this domain. All models and a subset of the SurgeNetXL dataset, including over 2 million video frames, are publicly available at: https://github.com/TimJaspers0801/SurgeNet.

==> Sections/1-Introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Barrett's Esophagus (BE) is a well-known precursor for Esophageal Adenocarcinoma (EAC), necessitating regular endoscopic surveillance for early detection and treatment, which has a good prognosis~\citep{ResectionPech,ResectionWeusten}. However, identifying early neoplastic changes in BE is challenging due to the subtle endoscopic appearance of lesions, characterized by only minimal mucosal and vascular changes~\citep{BORN,SubtletyScholvinck}, and the potential for sampling errors from extensive random biopsy protocols~\citep{Sampling}. Although modern endoscopes can visualize most subtle mucosal and vascular changes, the detection of neoplasia largely depends on the ability of the endoscopist to recognize these subtle features. Despite correct identification, the subtle nature of lesions often causes endoscopists to struggle with optimal biopsy placement for pathological confirmation, potentially leading to understaging of the disease status or missed neoplasia. These limitations underscore the potential utility of Computer-Aided Detection (CADe) systems in assisting endoscopists with the identification and localization of early neoplastic lesions.  

Several Computer-Aided Detection (CADe) systems for Barrett's neoplasia have been developed, to assist endoscopists in recognizing neoplastic lesions~\citep{Ebigbo,DeGroof,Hashimoto,Hussein,FockensBE2,Abdelrahim,Meinikheim}, which have proven to be an effective assistive tool to enhance detection rates of endoscopists~\citep{FockensBE2}. The developments of these systems necessitate numerous design decisions to effectively address the task's inherent complexities. Among these, the most critical choice is the choice of network architecture. Convolutional Neural Networks (CNNs) have traditionally been the state-of-the-art in various computer vision (CV) applications and the preferred architecture for Barrett's neoplasia detection~\citep{FockensBE2,Abdelrahim,Meinikheim}. However, recent advancements have introduced novel architectures that challenge the dominance of CNNs. The Vision Transformer (ViT)~\citep{ViT} and its derived instances, collectively known as Transformers, have rapidly gained prominence, offering competitive performance with CNNs. While the potential impact of Transformers on medical image analysis~\citep{ReviewShamshad,ReviewAzad} is still under investigation, particularly in gastrointestinal image analysis~\citep{KustersAMAI}~\hlnew{\citep{KustersMEDIA}}, hybrid architectures combining CNNs and Transformers have begun to emerge, aiming to leverage the strengths of both approaches. More recently, a new class of vision backbones utilizing State-Space Models (SSMs) have been introduced~\citep{ViM}, based on the Mamba deep learning model, which has shown great potential for long-sequence modeling while offering sub-quadratic complexity~\citep{Mamba}. These recent advancements highlight the need for careful consideration of architectural choices in developing CADe systems for Barrett's neoplasia detection, since each architecture presents distinct features and limitations that can significantly impact system performance and clinical utility. 

Another critical aspect of this task is the inherent variability in endoscopic image quality, which can often be compromised by artifacts such as motion and/or focus blur and improper lighting conditions, resulting in/from suboptimal imaging. Additionally, the visual characteristics of endoscopic images can vary significantly depending on the acquisition device, influenced by inherent post-processing and compression steps. Studies have demonstrated that the performance of deep learning-based techniques is highly sensitive to the quality and appearance of input images; even minor degradations can result in a significant performance decline~\citep{HendrycksRobustness,PeiRobustness}. Our previous work has specifically highlighted these challenges within the context of endoscopic imagery~\citep{Jaspers-MEDIA}, and examined the robustness and generalization capabilities of CNNs and Transformers under application-specific conditions~\citep{KustersAMAI}~\hlnew{\citep{KustersMEDIA}}. For deep learning-based CADe systems to be effective in safety-critical applications, such as gastrointestinal cancer screening, additional aspects are important, such as robustness and generalization across diverse clinical scenarios. This requirement is particularly pressing due to the challenges posed by variations in image quality and appearance, which create a significant \emph{domain gap} when these systems are applied to the heterogeneous data found in real-world clinical practice. Ensuring reliable operation in clinical environments implies that these models can handle diverse and imperfect data. This would even allow video data of lower quality included in the database to improve robustness. Consequently, it is essential to evaluate and consider several training and inference strategies to enhance endoscopy-specific model robustness and generalization. Key strategies include careful architecture choice, in-domain pre-training~\citep{Jaspers-MEDIA,BoersMEDIA}, domain-specific augmentations and the incorporation of lower-quality video frames. 

% careful architecture choice, in-domain pre-training --> clinical GastroNet

Lastly, endoscopist compliance with CADe systems is often suboptimal due to inconsistent predictions and inaccurate localization, resulting in a joint sensitivity that is lower than the standalone CADe performance~\citep{FockensBE2}. CADe systems are designed to detect neoplastic lesions through binary classification and localization, requiring pixel-level annotations from Barrett's experts. However, the subtlety of these lesions can lead to significant inter-observer variability among experts resulting in inconsistent delineations of neoplasia~\citep{BoersCaption}. Incorporating this variability during training may help capture a broader spectrum of atypical neoplastic patterns, which is crucial for detecting particularly subtle variants. To enhance endoscopist compliance, it is essential to improve the localization and gradual neoplasia coverage of CADe systems, while consistency of predictions is a key factor. Therefore, it is vital to evaluate training and inference strategies that aim to enhance both the localization capabilities and the consistency of CADe predictions. 

This study aims to provide valuable insights into the design decisions of the structured development of CADe systems for Barrett's neoplasia detection, given the challenges inherent to the application and task. In summary, the paper presents several key contributions to the field, as listed below.
\begin{itemize}

\item[$\circ$] \emph{An in-depth evaluation of architectural choices, training strategies, and inference approaches} to offer comprehensive insights for a structured design of effective CADe systems for Barrett's neoplasia detection. This evaluation specifically addresses the unique challenges and complexities associated with endoscopic imaging and the nature of Barrett's neoplasia. 

\item[$\circ$] \emph{Measurable and incremental performance improvements} realized by the incorporation of structured design considerations into the development of CADe systems.

\item[$\circ$] \emph{A rigorous benchmark of the proposed architecture} against 6 state-of-the-art CADe systems for Barrett's neoplasia detection. The obtained results demonstrate that the proposed model achieves statistically significant improvements over existing systems in both classification and localization tasks, in terms of peak performance, generalization, and robustness, across 9 diverse test sets reflecting real-world clinical challenges.

\end{itemize}

The previous discussions have already summarized the multi-faceted nature of robust detection of BE neoplasia. Therefore, the data should contain sufficient diversity and quality variations to address robustness. This implies why we have adopted a hybrid CNN-Transformer solution, as it enables to jointly exploit the strengths of both architecture types. Another essential aspect for performance improvement coupled with robustness is to optimize training procedures. Therefore, the adopted solution is to employ large-scale domain-specific pre-training with a self-supervised learning objective on gastrointestinal data only. This training solution allows a larger number of data points to be included to learn characteristics of the gastrointestinal tract without requiring rigid annotation procedures. The previous aspects are found most relevant, but the remaining training and inference approaches offer notable additional interesting details that will be elaborated in this study, but not addressed here.

The remainder of the paper is organized as follows. Section~\ref{sec: RelatedWork} provides an overview of the related work. Section~\ref{sec: MaterialsMethods} describes the methods and materials used in this study. Section~\ref{sec: ExperimentalSetup} outlines the experiments conducted, while Section~\ref{sec: ResultsDiscussion} presents and extensively discusses the experimental results. Finally, Section~\ref{sec: Conclusions} presents the conclusions of this work.


==> Sections/2-RelatedWork.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RELATED WORK %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Barrett's CADe %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Barrett's neoplasia detection}
Numerous studies on deep learning-based CADe systems for Barrett's neoplasia detection have been documented in literature, showcasing a variety of CNN-based approaches and methodologies. For instance, Hashimoto~\textit{et al.}~\citep{Hashimoto} proposed a two-step algorithm, beginning with an Xception network for binary classification to assess the presence of neoplastic lesions, followed by object detection using YOLOv2 to detect and localize the neoplasia in positively identified frames, adopting an object detection strategy rather than a segmentation approach. Similarly, Hussein~\textit{et al.}~\citep{Hussein} and Abdelrahim~\textit{et al.}~\citep{Abdelrahim} employed separate networks for detection/classification and localization. Hussein~\textit{et al.}~\citep{Hussein} utilized a ResNet-101 architecture for neoplasia detection and an FCNResNet-50 architecture for neoplasia localization, while Abdelrahim~\textit{et al.}~\citep{Abdelrahim} implemented a VGG-16-based neoplasia detection model and a SegNet-based localization model. In contrast, other approaches have leveraged encoder-decoder architectures. Ebigbo~\textit{et al.}~\citep{Ebigbo} and Meinikheim~\textit{et al}~\citep{Meinikheim} used ResNet-101 and ResNet-50 encoders, respectively, paired with a DeepLabV3+ decoder. De Groof~\textit{et al.}~\citep{DeGroof} built upon the custom hybrid ResNet-UNet model~\citep{PuttenWLE}, while Fockens~\textit{et al.}~\citep{FockensBE2} introduced a quantized int8-based EfficientNet-lite1 architecture paired with a MobileNetV2-DeepLabV3+ decoder, emphasizing efficient integration into existing endoscopy systems. A significant gap exists in addressing the specific requirements of endoscopic applications, such as robustness and generalization to variable image quality, and advances in network architectures. However, Hussein~\textit{et al.}~\citep{Hussein} and Fockens~\textit{et al.}~\citep{FockensBE2} have proposed video-based models, consequently dealing with the lack of guarantees about the endoscopic video quality. De Groof~\textit{et al.}~\citep{DeGroof} and Fockens~\textit{et al.}~\citep{FockensBE2} have made preliminary steps towards domain-specific pre-training using semi-supervised learning, demonstrating increased model performance. 

While significant progress has been made in the development of deep learning-based CADe systems, current research still lacks comprehensive strategies for the structured design of these systems, particularly in enhancing robustness, generalization, and proper evaluation of these critical aspects. Deep learning models are particularly susceptible to challenges related to the variability in endoscopic image quality and appearance~\hlnew{\citep{KustersMEDIA}}~\citep{Jaspers-MEDIA}, highlighting the need for further exploration and refinement in these areas. To enhance the practical applicability and reliability of CADe systems across diverse clinical settings, it is essential to incorporate rigorous development methodologies and thorough evaluations that specifically address the complexities and variability inherently captured in real-world clinical data.


==> Sections/3-MaterialsMethods.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATERIALS AND METHODS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This study aims to shed some light on the design choices for the structured development of CADe systems for Barrett's neoplasia detection, for which the material and methodology are described in the upcoming subsections. First, Section~\ref{sec: MaterialsMethods-Data} provides a detailed description of the datasets employed in the various experiments. Subsequently, in Section~\ref{sec: MaterialsMethods-Pre-process} the data pre-processing techniques are discussed, followed by an explanation of the training procedure and description of the performance evaluation in Sections~\ref{sec: MaterialsMethods-TrainingDetails} and~\ref{sec: MaterialsMethods-Evaluation}, respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: DATASETS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data}
\label{sec: MaterialsMethods-Data}

\subsubsection{Data acquisition}
Data for algorithm development and evaluation are sourced from both internal and external collections. Internally, a set of private data are collected, comprising both retrospective and prospective data, from 15~international participating centers of the BONS-AI consortium (Barrett's OesophaguS imaging for Artificial Intelligence). All data are acquired using Olympus gastroscopes (Olympus Corp., Tokyo, Japan), and include imagery of Barrett's neoplasia and non-dysplastic BE (NDBE), with histopathology confirmation through biopsy or resection. Data concerning Barrett's neoplasia detection are captured using White Light Endoscopy (WLE), wherein prospective material is recorded without a specific focus on neoplastic lesions, if present. De-identification procedures align with the General Data Protection Regulation (EU) 2016/679. A detailed description of the data acquisition protocol has been published elsewhere~\citep{FockensBE2,FockensBE}.

%
\begin{table*}[t]
\caption{Description of datasets used for CADe algorithm development and evaluation for the Barrett's neoplasia detection task. Number of images/frames with corresponding number of patients for the algorithm development, peak performance, generalization and robustness evaluation test sets. GT masks contain data with expert annotations used for localization performance for lesions.}
\centering
\begin{tabular}{l | c c c | c }
\toprule
\textbf{Dataset} & \textbf{NDBE} & \textbf{BE neoplasia} & \textbf{Total} & \textbf{GT masks} \\
\midrule
\textcolor{gray}{\textit{Development data}} & & & & \\
  Training~~~~~~\textit{Images}             & 7,595\pt{1,095}         & 6,251\pt{1,296}     & 13,846\pt{2,391}      & 2,752 \\
  ~~~~~~~~~~~~~~~~~~~\textit{HQ Frames}     & 1,621 ~~~\pt{98}        & 1,505 ~~~\pt{86}    & ~~3,126 ~\pt{184}     & ~~~~~~~/   \\
  ~~~~~~~~~~~~~~~~~~~\textit{MQ Frames}     & 1,855 ~~~\pt{99}        & 1,835 ~~~\pt{96}    & ~~3,690 ~\pt{195}     & ~~~~~~~/   \\
  ~~~~~~~~~~~~~~~~~~~\textit{LQ Frames}     & 1,084 ~~~\pt{85}        & ~~~872 ~~~\pt{72}   & ~~1,956 ~\pt{157}     & ~~~~~~~/   \\
  Validation ~\textit{Images}               & ~~~100 ~~~\pt{36}       & ~~~100 ~~~\pt{58}   & ~~~~~200 ~~~\pt{94}   & ~~~~~96   \\
  ~~~~~~~~~~~~~~~~~~\textit{HQ Frames}      & ~~~543 ~~~\pt{27}       & ~~~473 ~~~\pt{36}   & ~~1,016 ~~~\pt{63}    & ~~~~~~~/   \\
  ~~~~~~~~~~~~~~~~~~\textit{MQ Frames}      & ~~~533 ~~~\pt{28}       & ~~~537 ~~~\pt{39}   & ~~1,070 ~~~\pt{67}    & ~~~~~~~/   \\
  ~~~~~~~~~~~~~~~~~~\textit{LQ Frames}      & ~~~390 ~~~\pt{23}       & ~~~280 ~~~\pt{32}   & ~~~~~670 ~~~\pt{55}   & ~~~~~~~/   \\
 \midrule
 \midrule
 \textcolor{gray}{\textit{Peak performance test sets}} & & & &  \\
 BM Test                  & ~~~300 ~\pt{125}       & ~~~100 ~~~\pt{50}      & ~~~~~400 ~\pt{175}            & ~~~100   \\
 AC Test                  & ~~~327 ~~~\pt{73}      & ~~~~~82 ~~~\pt{46}     & ~~~~~409 ~\pt{119}            & ~~~~~82   \\
 \midrule
 \textcolor{gray}{\textit{Generalization test sets}} & & & & \\
 ARGOS DS 3+4             & ~~~208 ~~~\pt{81}      &  ~~~169 ~~~\pt{94}     & ~~~~~377 ~\pt{175}            & ~~~169   \\
 ARGOS DS 5               &  ~~~~~40 ~~~\pt{40}    &  ~~~~~40 ~~~\pt{40}    & ~~~~~~~80 ~~~\pt{80}          & ~~~~~40  \\
 BORN                     & ~~~254 ~~~\pt{32}      &  ~~~124 ~~~\pt{64}     & ~~~~~378 ~~~\pt{96}           & ~~~124   \\
\midrule
 \textcolor{gray}{\textit{Robustness test sets}} & & & &  \\
 IQ Triplet               & ~~~168 ~~~\pt{50}      & ~~~183 ~~~\pt{53}      & ~~~~~351 ~\pt{103}            & ~~~~~~~/  \\
 BM Test-C                & 1,500 ~\pt{125}        & ~~~500 ~~~\pt{50}      & ~~2,000 ~\pt{175}             & ~~~500   \\
\bottomrule
\end{tabular}
\label{table: MaterialsMethods-Data-CADe Datasets}
\end{table*}
%


%
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/Endoscopy/EndoscopyImageryV2.pdf}
    \caption{Variational samples of the different test sets for the Barrett's neoplasia detection task; (a) BM Test: NDBE case; (b) AC Test: evident neoplastic case; (c) BM Test: subtle neoplastic case; (d) ARGOS DS 3+4: NDBE case from different scope manufacturer; (e) ARGOS DS 3+4: evident neoplastic case from different scope manufacturer; (f) ARGOS DS 5: subtle neoplastic case from different scope manufacturer; (g) BORN: NDBE case of overall lower quality from older generation scope; (h) BORN: evident neoplastic case of overall lower quality from different scope manufacturer; (i)-(l) BM Test-C: degraded versions of (c). Corrupted hue and motion blur; corrupted saturation and overexposure; overexposure, motion blur, corrupted hue and brightness; overexposure, motion blur and corrupted hue and brightness; (m)-(o) IQ Triplet: neoplastic case in HQ, MQ with motion blur and underexposure, and LQ with severe overexposure; (p)-(r) IQ Triplet: NDBE case in HQ, MQ with motion blur, and LQ with severe underexposure.}
    \label{fig: MaterialsMethods-Data-ExampleImages}
\end{figure*}
%


\subsubsection{Datasets}
\label{sec: MaterialsMethods-Data-CADeDatasets}

\indent {\textsc{A. Training and validation sets}: The dataset utilized for algorithm development consists of a training and validation set sourced from the internal BONS-AI dataset, with the validation set used for hyper-parameter tuning and model checkpoint selection. Additionally, videos are available for a subset of prospectively recorded patients, curated for neoplastic lesion visibility, if present. An in-house tool is employed to sample \emph{key frames} from these videos, taking into account image quality and semantic information, resulting in three sets of video frames (HQ, MQ and LQ) based on predefined quality thresholds. For each video in the training and validation set, a maximum of~10 and 5~key frames are sampled, respectively. The impact of incorporating sampled frames as a supplement to the default training set is evaluated in the experiments discussed in Sections~\ref{sec: ExperimentalSetup-Training-VideoFrames} and~\ref{sec: ResultsDiscussion-Training-VideoFrames}. Moreover, the high-quality frames (HQ) of the validation set are combined with the validation images, to enhance the size and consequently the resolution of the validation set used for hyper-parameter tuning, checkpoint selection of the model and performance comparison among models. Furthermore, the MQ and LQ frames of the validation set are leveraged for post-training validation concerning model robustness, as these resemble lower-quality imagery encountered in clinical practice. The representativeness of cases in the training and validation set is ensured by clinical guidance. Additionally, a strict patient-based split between training, validation and all test sets is employed to mitigate data leakage and intra-patient bias. A detailed summary of algorithm development sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets}.

% The datasets utilized for algorithm development consist of a training and validation set sourced from the internal BONS-AI dataset. The training set consists of 13,846~images (2,391~patients), containing 6,251~neoplastic images (1,296~patients) and 7,595~NDBE images (1,095~patients). The validation set used for hyper-parameter tuning and model checkpoint selection comprises of 200~images (94~patients), containing 100~neoplastic images (58~patients) and 100~NDBE images (36~patients). Additionally, videos are available for a subset of prospectively recorded patients, curated for neoplastic lesion visibility, if present. An in-house tool is employed to sample \emph{keyframes} from these videos, taking into account image quality and semantic information, resulting in three sets of video frames (HQ, MQ and LQ) based on predefined quality thresholds. The video training set included 304~neoplastic videos (99~patients) and 311~NDBE videos (99~patients), while the video validation set comprises 183~neoplastic videos (39~patients) and 196~NDBE videos (28~patients). For each video in the training and validation set, a maximum of 10 and 5 keyframes are sampled, respectively. The impact of incorporating sampled frames as a supplement to the default training set is evaluated in the experiments discussed in Sections~\ref{sec: ExperimentalSetup-Training-VideoFrames} and~\ref{sec: ResultsDiscussion-Training-VideoFrames}. Moreover, the high quality (HQ) frames of the validation set are combined with the validation images, to enhance the size and consequently the resolution of the validation set used for hyper-parameter tuning, model checkpoint selection and performance comparison among models. Furthermore, the MQ and LQ frames of the validation set are leveraged for post-training validation concerning model robustness, as these resemble lower-quality imagery encountered in clinical practice. Representativeness of cases in the training and validation set is ensured by clinical guidance. Additionally, a strict patient-based split between training, validation and all test sets is employed to mitigate data leakage and intra-patient bias. A detailed summary of algorithm development sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets}.

\indent \textsc{B. Peak performance test sets}: To evaluate peak performance, two independent test sets derived from the internal BONS-AI dataset are considered. Firstly, the benchmarking test set (BM Test) reflects the most challenging cases for endoscopists in clinical practice, which is artificially enriched with subtle neoplastic cases. Secondly, the all-comers test set (AC Test) represents the spectrum of cases encountered in routine clinical practice, which consists of consecutive cases recorded prospectively at participating centers over a two-month period. A detailed summary of peak performance evaluation sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets} and example images are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This approach ensures thorough evaluation across challenging scenarios and real-world clinical settings, providing robust insights into algorithm performance.

% To evaluate peak performance, two independent test sets derived from the internal BONS-AI dataset are considered. Firstly, the benchmarking test set (BM Test) comprises 400~images (175~patients), featuring 100~neoplastic images (50~patients) and 300~NDBE images (125~patients). The BM Test set is artificially enriched with subtle neoplastic cases to reflect the most challenging cases for endoscopists in clinical practice. Secondly, the all-comers test set (AC Test) comprises 409~images (119~patients), including 82~neoplastic images (46~patients) an 327~NDBE images (73~patients). The AC Test set consists of consecutive cases recorded prospectively at participating centers over a two-month period, thus representing the spectrum of cases encountered in routine clinical practice. A detailed summary of peak performance evaluation sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets} and example images are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This approach ensures thorough evaluation across challenging scenarios and real-world clinical settings, providing robust insights into algorithm performance.

\indent \textsc{C. Generalization test sets}: To assess generalization performance, three distinct external datasets are employed. Firstly, the BORN test set which was extracted from videos within the BORN training module~\citep{BORN}. These videos were retrospectively collected from 3~international centers, employing Olympus (Olympus Corp., Tokyo, Japan) and Fujifilm (Fujifilm Corp., Japan) gastroscopes. Notably, the Olympus gastroscopes utilized in the acquisition belong to older generations compared to those used in our internal data collection, therefore providing imagery with lower objective quality. 
Secondly, the data from the ARGOS project~\citep{DeGroof,ARGOS1} was leveraged to form two additional test sets, acquired exclusively with Fujifilm gastroscopes. Dataset~3 of the ARGOS project was prospectively collected from 2~centers in The Netherlands, while Dataset~4 was retrospectively collected from 4~international centers. The ARGOS Datasets~3 and~4 were combined to constitute one of the generalization test sets (ARGOS DS~3+4), which presents a heterogeneous dataset in terms of lesion subtlety. Furthermore, Dataset~5 from the ARGOS project is employed as an independent test set, prospectively gathered from 4~international centers. This dataset (ARGOS DS~5) was intentionally enriched with subtle neoplastic lesions, posing a greater detection and delineation challenge. A detailed summary of the generalization test sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets} and example images are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This comprehensive approach with three test sets ensures thorough evaluation across scenarios characterized by varying objective image quality and diverse data sources, including older generation scopes and/or different manufacturers. The assessment encompasses general, more evident, lesions as well as especially subtle neoplastic lesions, thereby furnishing robust insights into the generalization performance and performance on challenging cases.

% To assess generalization performance, two distinct external datasets are employed. Firstly, the BORN test set was extracted from videos within the BORN training module~\citep{BORN}. These videos were retrospectively collected from 3~international centers, employing Olympus (Olympus Corp., Tokyo, Japan) and Fujifilm (Fujifilm Corp., Japan). Notably, the Olympus gastroscopes utilized in the acquisition belong to older generations compared to those used in our internal data collection, therefore resulting in imagery with lower objective quality. The BORN test set comprises 378~images (96~patients), including 124~neoplastic images (64~patients) and 254~NDBE images (32~patients). 
% Secondly, the data from the ARGOS project~\citep{DeGroof,ARGOS1} was leveraged to form two additional test sets, acquired exclusively with Fujifilm gastroscopes. Dataset~3 of the ARGOS project was prospectively collected from 2~centers in The Netherlands, while Dataset~4 was retrospectively collected from 4~international centers. The ARGOS Datasets 3 and 4 were combined to constitute one of the generalization test sets (ARGOS DS~3+4), which presents a heterogeneous dataset in terms of lesion subtlety, and comprises 377~images (175~patients), including 169~neoplastic images (94~patients) and 208~NDBE images (81~patients). Furthermore, Dataset~5 from the ARGOS project is employed as an independent test set, prospectively gathered from 4~international centers. This dataset (ARGOS DS~5) was intentionally enriched with subtle neoplastic lesions, posing a greater detection and delineation challenge. ARGOS DS~5 comprises 80~images (80~patients), including 40~neoplastic images (40~patients) and 40~NDBE images (40~patients). A detailed summary of the generalization test sets is presented in Table~\ref{table: MaterialsMethods-Data-CADe Datasets} and example images are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This comprehensive approach with three different test sets ensures thorough evaluation across scenarios characterized by varying objective image quality and diverse data sources, including older generation scopes and different manufacturers. The assessment encompasses general, more evident, lesions as well as especially subtle neoplastic lesions, thereby furnishing robust insights into the generalization and challenging-case performance. 

\indent \textsc{D. Robustness test sets}: To evaluate robustness, two distinct test sets are considered, derived from the internal BONS-AI dataset. Firstly, a test set (IQ Triplet) is constructed that includes images spanning the full range of endoscopic image quality, representing the spectrum encountered in real-world scenarios. This spectrum includes high-quality images captured by expert endoscopists in tertiary referral centers to low-quality images encountered in routine clinical practice. Endoscopic image quality can be affected by several factors, however, this test set specifically focuses on endoscopist-dependent image quality parameters such as esophageal expansion, lighting conditions, blurriness and degree of esophageal cleaning. For each patient/lesion, a matched triplet of video frames was collected by a dedicated clinical research fellow and consequently confirmed by a Barrett's expert. This process yielded three subsets based on distinct levels of image quality: high (HQ), moderate (MQ) and low-quality (LQ) test sets.
Secondly, the original BM Test set is corrupted with clinically realistic and calibrated synthesized corruptions for endoscopic imagery. Specifically, by defining three user-dependent corruptions (motion blur, local focus blur and overexposure), five image acquisition and processing corruptions (contrast, saturation, hue, brightness and sharpness) and three compression artifacts (JPEG compression, JPEG2000 compression and resolution reduction). The corrupted BM Test set (BM Test-C) is created by randomly applying up to five corruptions with random severity levels to each image simultaneously, within realistic clinically calibrated ranges. This process is repeated five times, resulting in a set that is five times larger than the original BM Test set. Detailed information and technical details about the generation of corruptions are described in our previous work~\citep{Jaspers-MEDIA,RobustnessTool-JaspersAMAI}. Some example images for the paired test set and the BM Test-C set are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This approach facilitates a direct and comprehensive evaluation of robustness, comparing the performance between clean, high-quality images and corrupted, low-quality versions within the respective test sets. This evaluation encompasses both real-world variations and artificially induced image corruptions, providing a thorough assessment of clinically relevant robustness.


% To evaluate robustness, two distinct test sets derived from the internal BONS-AI dataset are considered. Firstly, a test set (IQ Triplet) is constructed that includes images spanning the full range of endoscopic image quality, representing the spectrum encountered in real-world scenarios. This spectrum includes high-quality images captured by expert endoscopists in tertiary referral centers to lower quality images encountered in routine clinical practice. Endoscopic image quality can be affected by several factors, however, this test set specifically focuses on endoscopist-dependent image quality parameters such as esophageal expansion, lighting conditions, blurriness and degree of esophageal cleaning. For each patient/lesion, a matched triplet of video frames was collected by a dedicated clinical research fellow and consequently confirmed by a Barrett's expert. This process yielded three subsets based on distinct levels of image quality: high (HQ), moderate (MQ) and low-quality (LQ) test sets. The total IQ Triplet test set comprises 351~images (103~patients), including 183~neoplastic images (53~patients) and 168~NDBE images (50~patients), resulting in 61~neoplastic and 56~NDBE images in each of the subsets.   
% Secondly, the original BM Test set is corrupted with clinically realistic and calibrated synthesized corruptions for endoscopic imagery. Specifically, by defining three user-dependent corruptions (motion blur, local defocus blur and overexposure), five image acquisition and processing corruptions (contrast, saturation, hue, brightness and sharpness) and three compression artifacts (JPEG compression, JPEG2000 compression and resolution reduction). The corrupted BM Test set (BM Test-C) is created by randomly applying up to five corruptions with random severity levels, within realistic clinically calibrated ranges, to each image simultaneously. This process is repeated five times, resulting in 2,000~images for the BM Test-C set. Detailed information and technical details about the generation of corruptions is described in our previous work~\citep{Jaspers-MEDIA,RobustnessTool-JaspersAMAI}. Some example images for the paired test set and the BM Test-C set are depicted in Fig.~\ref{fig: MaterialsMethods-Data-ExampleImages}. This approach facilitates a direct and comprehensive evaluation of robustness, comparing the performance between clean, high-quality images and corrupted, low-quality versions within the respective test sets. This evaluation encompasses both real-world variations and artificially induced image corruptions, providing a thorough assessment of clinically relevant robustness.

\indent \textsc{E. Segmentation ground-truth creation}: For internal BONS-AI data, neoplasia delineations are obtained from 14~Barrett's experts, where at least 2~experts delineated the same image. For each image, the experts delineated the largest area atypical from normal NDBE, suspected to be neoplasia (Lower Likelihood, LL), and the area within it standing out more profoundly (Higher Likelihood, HL). To achieve a minimum level of consensus, a third expert endoscopist is invited in case the two HL delineations obtain less than 30\%~agreement in terms of Dice Score. Subsequently, the two delineations among the three experts that achieve the highest overlap are used for further ground-truth (GT) processing. Several consensus GT masks with increasing neoplastic certainty can be constructed: Soft-spot GT, Plausible-spot GT, Sweet-spot GT and Hard-spot GT, which are defined in Table~\ref{table: MaterialsMethods-Data-ConsensusGT}. For model training, also Average GT, Random GT and Multiple GT strategies are considered~\hlnew{\citep{Kusters-CaPTion-GTConsensus}}, also defined in Table~\ref{table: MaterialsMethods-Data-ConsensusGT}. An example case with GT masks is illustrated in Fig.~\ref{fig: MaterialsMethods-Data-GroundTruth}. The default choice as consensus GT mask for training and evaluation purposes is the Plausible GT, in line with our previous work~\citep{FockensBE2,FockensBE}. The remaining consensus GT variants are experimented with for training in experiments related to Sections~\ref{sec: ExperimentalSetup-Training-GT} and~\ref{sec: ResultsDiscussion-Training-GT}. For the BORN test set, neoplasia delineations were obtained from 4~Barrett's experts, where at least 3~experts delineated the same image. A consensus GT mask is constructed by the intersection of the three delineations.
For the ARGOS test sets, neoplasia delineations are obtained from 8~Barrett's experts, where at least~3 or 6~experts delineated the same image for ARGOS DS~3+4 and ARGOS DS~5, respectively. A consensus GT mask is constructed by the region that the majority of experts delineated as neoplastic (i.e. $\geq$ 2 or $\geq$ 4). The number of consensus GT masks for each dataset are specified in Table~\ref{table: MaterialsMethods-Data-CADe Datasets}.


% For internal BONS-AI data, neoplasia delineations are obtained from 14 Barrett's experts, where at least 2 experts delineated the same image. For each image, the experts delineated the largest area atypical from normal NDBE, suspected to be neoplasia (Lower Likelihood, LL), and the area within it that stands out more profoundly (Higher Likelihood, HL). To achieve a minimum level of consensus, a third expert endoscopist is invited in case the two HL delineations obtained less than 30\% agreement in terms of Dice Score. Subsequently, the two delineations among the three experts that achieve the highest overlap are used for further ground-truth (GT) processing. Several consensus GT masks with increasing neoplastic certainty can be constructed: Soft spot GT, Plausible spot GT, Sweet spot GT and Hard spot GT, which are defined in Table~\ref{table: MaterialsMethods-Data-ConsensusGT}. For model training, also Average GT, Random GT and Multiple GT strategies are considered \textcolor{red}{\textbf{MICCAI}}, also defined in Table~\ref{table: MaterialsMethods-Data-ConsensusGT}. An example case with GT masks is illustrated in Fig.~\ref{fig: MaterialsMethods-Data-GroundTruth}. The default choice as consensus GT mask for training and evaluation purposes is the Plausible GT, in line with our previous work~\citep{FockensBE2,FockensBE}. The remaining consensus GT masks are experimented with for training in experiments related to Sections~\ref{sec: ExperimentalSetup-Training-GT} and~\ref{sec: ResultsDiscussion-Training-GT}. For the training, validation, BM Test and AC Test there are 2,752, 96, 100 and 82 consensus GT masks available, respectively. For the BORN test set, neoplasia delineations were obtained from 4~Barrett's experts, where at least 3~experts delineated the same image. A consensus GT mask is constructed by the intersection of the three delineations, resulting in 124~GT masks. For the ARGOS test sets, neoplasia delineations are obtained from 8~Barrett's experts, where at least~3 or 6~experts delineated the same image for ARGOS DS 3+4 and ARGOS DS 5, respectively. A consensus GT mask is constructed by the region that the majority of experts delineated as neoplastic (i.e. $\geq$ 2 or $\geq$ 4), resulting in a total of 209~GT masks for the test sets combined.

%
\begin{table*}[t]
\caption{Definitions of GT strategies with consensus segmentation. Subscript indices for the $\text{LL}$ and $\text{HL}$ delineations correspond to the respective expert numbers.}
\centering
\begin{tabular}{l | c  c }
\toprule
\textbf{Consensus GT} \mbox{ } & \textbf{Definition} & \textbf{Description of delineations} \\
\midrule
 Soft-spot GT          & $\text{LL}_1 \cup \text{LL}_2$ & Areas delineated as neoplastic and/or atypical  \\ 
 Plausible-spot GT      & $(\text{LL}_1 \cap \text{LL}_2) \cup \text{HL}_1 \cup \text{HL}_2$ \mbox{ } & Areas delineated as neoplastic by $\geq$ 1 expert and atypical by both experts   \\
 Sweet-spot GT           & $\text{HL}_1 \cup \text{HL}_2$ & Areas delineated as neoplastic by $\geq$ 1 expert   \\
 Hard-spot GT           & $\text{HL}_1 \cap \text{HL}_2$ & Areas delineated as neoplastic by both experts \\
 \midrule
 Average GT & / & Averaged all consensus masks in single non-binary mask \\
 Random GT & / & Randomly sampling single consensus mask during training \\
 Multiple GT & / & Provide all consensus masks simultaneously during training \\
 
 % Average & \multicolumn{2}{l}{Averaged consensus masks in single non-binary mask} \\
 % Random & \multicolumn{2}{l}{Randomly sampling single consensus mask during training} \\
 % Multiple & \multicolumn{2}{l}{Provide all consensus masks during training} \\
 
\bottomrule
\end{tabular}
\label{table: MaterialsMethods-Data-ConsensusGT}
\end{table*}
%

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ground Truth/GroundTruth-cropped.pdf}

    \caption{Example lesion with delineations and consensus GTs for internal BONS-AI data. (a) Neoplastic lesion; thick green/blue lines indicate HL delineations, and thinner lines indicate LL delineations. (b)-(e) Corresponding consensus GT masks. (f) Consensus GT masks pooled into non-binary average map. (g) For Multiple GT all consensus masks are provided simultaneously. For Random GT one of (b)-(e) is sampled randomly in every iteration during training.}
    \label{fig: MaterialsMethods-Data-GroundTruth}
\end{figure*}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: DATA PRE-PROCESSING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data pre-processing}
\label{sec: MaterialsMethods-Pre-process}
The pre-processing of the data consists of several steps. Initially, the central active region of raw endoscopic images are resized to 256$\times$256~pixels. Subsequently, pixel-intensity values are normalized by channel-wise subtraction of the mean and division by the standard deviation, leveraging statistics derived from the training data. 
To improve generalization and virtually expand the dataset size, a variety of random data augmentation techniques are applied during training. The default \emph{non-domain-specific} augmentation (N-DSA) techniques encompass a range of fundamental transformations, including horizontal and vertical flipping, rotation, and adjustments to contrast, saturation, and brightness. Additionally, grayscale conversion, Gaussian blurring, random affine and sharpness transformations are applied, as well as randomly introducing artificial noise corruption. In contrast to the N-DSA techniques, a specialized set tailored to the endoscopy domain is defined. This set of \emph{domain-specific} augmentations (DSA) includes motion, zoom, lens, median and focus blur, along with hue enhancements. Moreover, selected techniques from the N-DSA set are utilized, albeit with calibrated parameter ranges to ensure generation of realistic augmentations pertinent to the nuances of the endoscopy domain. The N-DSA techniques are the standard choice for training and validation purposes. The DSA techniques are evaluated for training and validation in the experiments discussed in Sections~\ref{sec: ExperimentalSetup-Training-Augmentation} and~\ref{sec: ResultsDiscussion-Training-Augmentation}. Given the relatively limited size of the validation set, during validation steps an approach is adopted to ensure reliable performance estimation. Specifically, evaluation occurs four times on distinct randomly augmented validation sets, thereby providing a more reliable performance estimate. Further details are discussed in Appendix~\ref{sec: Supplementary-Preprocess}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: TRAINING DETAILS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training procedure}
\label{sec: MaterialsMethods-TrainingDetails}
The training framework for all experiments has employed the Adam optimizer with AMS-grad, incorporating a weight decay of 10$^{-4}$ and $(\beta_1, \beta_2)$ = (0.9, 0.999). Additionally, a dynamic learning rate scheduler is integrated that reduces the learning rate by a factor of~10 when the validation loss saturates for 10~epochs, with a maximum of 3~reductions. Moreover, an early stopping mechanism is implemented, that terminates the training procedure if there is no improvement larger than 0.05\% in validation performance for 25~epochs. For the experiments, learning rates within the range of [10$^{-4}$, 10$^{-6}$] are utilized. For the classification task, the Binary Cross-Entropy (BCE) loss is employed. For segmentation tasks, a composite function combining BCE and Dice loss is used as the default choice. However, in the experiments discussed in Sections~\ref{sec: ExperimentalSetup-Training-GT} and~\ref{sec: ResultsDiscussion-Training-GT}, where Average GT and Multiple GT are used during training, there are deviations from this default choice. For Average GT, BCE is used as the segmentation loss because Dice is only suitable for binary GT masks. For the Multiple GT strategy, the composite BCE+Dice loss is extended to compute the average loss between the predicted segmentation mask and the four individual consensus GT masks, \hlnew{in line with our previous work~\citep{Kusters-CaPTion-GTConsensus}}. To enhance model generalization, label smoothing of~0.01 is employed across all loss functions. Despite the absence of ground-truth delineations in some neoplastic images, their inclusion significantly contributes the training of the backbone encoder in multi-task learning, by leveraging backpropagation of the classification loss which involves the classification label. To ensure balanced representation during training, random sampling is employed that maintains an average 50-50\% distribution of classes in each iteration. All experiments are conducted across five distinct training cycles, each initiated with unique random seeds. All implementations are performed in Python using PyTorch (Lightning) frameworks and are executed on 40-GB A100 GPUs (NVIDIA Corp., CA, USA).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: PERFORMANCE EVALUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance evaluation}
\label{sec: MaterialsMethods-Evaluation}

\subsubsection{Metrics}
The performance of the models is evaluated based on their ability to perform classification, classification-by-segmentation and localization. To assess the classification performances of a model, the Area Under the Receiver Operating Characteristic (AUROC) and Precision-Recall Curve (AUPRC) are used. The AUROC provides a comprehensive summary of the model's sensitivity and specificity, while the AUPRC provides a comprehensive summary of the model's precision and recall. The AUROC and AUPRC values are calculated based on the output of the classification branch and the maximal pixel value in the segmentation prediction together with the corresponding GT label, for the classification (AUROC$_{cls}$/AUPRC$_{cls}$) and segmentation (AUROC$_{seg}$/AUPRC$_{seg}$) branch, respectively. To evaluate the localization performance on images with a GT mask, the mean Dice Score ($mD_i$) is employed. This metric measures the overlap between the predicted segmentation mask and the GT mask, thresholded by~0.5. 


\subsubsection{Statistical analysis}
To ensure robust conclusions in the comparative analysis of the proposed CADe model and state-of-the-art models for Barrett's neoplasia detection, statistical testing is essential. In this study, the Wilcoxon signed-rank test~\citep{Wilcoxon} is applied to assess the significance of differences in evaluation metrics across multiple test sets and metrics between the models. This non-parametric test is particularly well-suited for paired sample comparisons and is recommended by Rainio~\textit{et al.}~\citep{RainioStats} as a preferred alternative to the Friedman's test~\citep{Friedman}, especially given the relatively small number of test sets involved (despite the inclusion of several models). The Wilcoxon test is applied between the proposed CADe model and each state-of-the-art comparator model. To mitigate the risk of Type-I errors due to multiple comparisons, the Benjamini-Hochberg~\citep{Benjamini-Hochberg} procedure is utilized for a correction of multiple testing. By performing the Wilcoxon test for each evaluation metric across all test sets and for combinations of test sets across all metrics, a comprehensive comparison is ensured. 

% In this study, the Friedman's test~\citep{Friedman} is employed to evaluate the significance of differences across multiple models. This non-parametric test, particularly suited for analyzing paired samples, is recommended by Rainio~\textit{et al.}~\citep{RainioStats} as a preferred alternative to the Wilcoxon signed-rank test~\citep{Wilcoxon} when comparign several models. Friedman's test provides as single $p$-value, indicating whether significant differences exists among all the models under comparison. To assess which specific pairs of models exhibit significant differences, the Nemenyi post-hoc test~\citep{Nemenyi} is subsequently applied. This combination of Friedman's test and the Nemenyi post-hoc test is systematically performed for each evaluation metric across all test sets, ensuring a comprehensive comparison.


==> Sections/4-Experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section provides a comprehensive overview of the experiments conducted to evaluate design choices for the structured development of a CADe system for Barrett's neoplasia detection. Each subsection focuses on a specific design choice, detailing the corresponding experimental setup. Firstly, Section~\ref{sec: ExperimentalSetup-Backbone} offers an in-depth description of the selected backbone architectures for comparison, which is followed by a description of the semantic segmentation decoder architectures considered in our study in Section~\ref{sec: ExperimentalSetup-Decoder}. Next, Section~\ref{sec: ExperimentalSetup-Training} explores various training strategies, including domain-specific pre-training, data augmentation, training with additional video frames, and the utilization of segmentation GT. Then Section~\ref{sec: ExperimentalSetup-Inference} outlines several inference strategies, such as considerations in how to use model output and TensorRT conversion~\citep{TensorRT}. The complete section is concluded  in Section~\ref{sec: ExperimentalSetup-SOTA} with a description of the state-of-the-art methods against which the proposed approach is benchmarked. A graphical summary of the series of experiments is depicted in Fig.\ref{fig: ExperimentalSetup}.

%
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Infographic/experimental_setup-cropped.pdf}

    \caption{Graphical representation of the series of experiments, with corresponding section numbers provided for each set of experiments, indicating where the experimental procedures are described and the results discussed.}
    \label{fig: ExperimentalSetup}
\end{figure*}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Model backbone selection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model backbone selection}
\label{sec: ExperimentalSetup-Backbone}
The process of selecting the backbone for the CADe model involves a rigorous comparative analysis encompassing ten deep learning architectures. These architectures are classified into four categories: pure Convolutional Neural Networks (CNNs), Transformer-based networks, Hybrid CNN-Transformer networks and State-Space Models (SSMs). The selected architectures represent a blend of established methodologies and cutting-edge advancements, ensuring a thorough exploration of the state-of-the-art in computer vision for the CADe framework. The selection of all network architectures is consistent within the range of parameter count typically associated with popular widely employed models such as ResNet-50 and ViT-S/16, to ensure that models are comparable in complexity. All backbone networks are initialized with ImageNet-pre-trained weights~\citep{ImageNet} and a simple classification head is attached after the final backbone feature extraction layer, consisting of a single output neuron followed by a Sigmoid activation function. A summary and comparison of the considered architectures, including parameters and model size, are provided by Table~\ref{table: ExperimentalSetup-SOTA CV Encoders}. The following subsections briefly discuss the indicated categories.

\subsubsection{Convolutional Neural Networks}
Among the CNNs considered is the well-established ResNet~\citep{ResNet} architecture, alongside newer advancements including ConvNeXt~\citep{ConvNeXt} and ConvFormer~\citep{MetaFormerBaselines}. The family of ConvNeXt models have emerged from modernizing the standard ResNet architecture towards the Vision Transformer (ViT)~\citep{ViT} design. Conversely, ConvFormer draws inspiration from the abstracted MetaFormer~\citep{MetaFormerBasic} approach, which prioritizes the overarching architecture of transformers over the specific token mixer mechanism (e.g. self-attention), considering it more pivotal for the model's performance. In ConvFormer, depth-wise separable convolution is the employed token mixer. 

\subsubsection{Hybrid CNN-Transformer}
For the hybrid architecture selection, recent innovations such as Inception Transformer (iFormer)~\citep{iFormer}, Unified transFormer (UniFormer)~\citep{UniFormerConference,UniFormerJournal} and \hlrev{CAFormer}~\citep{MetaFormerBaselines} are considered. Similar to ConvFormer, both iFormer and \hlrev{CAFormer} built upon the concept of the abstracted MetaFormer~\citep{MetaFormerBasic} approach. In iFormer, the Inception token mixer is introduced, which incorporates a channel-splitting mechanism to facilitate parallel convolution/max-pooling paths and a self-attention path, serving as high-frequency and low-frequency mixers, respectively. Similarly, \hlrev{CAFormer} leverages depth-wise separable convolutions in its lower stages, akin to ConvFormer, while employing vanilla self-attention in the upper stages. UniFormer distinguishes itself by introducing a versatile Relation Aggregator that seamlessly integrates convolution and self-attention for token-relation learning, achieving local and global token affinity. 

\subsubsection{Transformer}
The selection of native transformer architectures includes the vanilla ViT~\citep{ViT}, Pyramid Vision Transformer V2 (PVT)~\citep{PvTv2} and Swin Transformer V2 (Swin)~\citep{SwinV2}. Both PVT and Swin diverge from the vanilla ViT by integrating a hierarchical multi-scale pyramid structure. PVT adopts a progressive shrinking strategy to regulate the scale of feature maps through patch-embedding layers, while Swin incorporates patch-merging layers to generate a hierarchical feature representation. Additionally, Swin conducts self-attention within local, non-overlapping windows using shifted window partitioning across successive blocks. 

\subsubsection{State-space model}
Vision Mamba (Vim)~\citep{ViM} represents the category of State-Space Models. Vim is an extension of the Mamba deep learning model~\citep{Mamba} to the vision domain, which is an SSM with efficient hardware-aware design and significant potential for long-sequence modeling in NLP tasks, while offering sub-quadratic complexity. Vim incorporates bidirectional SSMs for data-dependent global visual context modeling and position embeddings for location-aware visual understanding.

%
\begin{table}[t]
\centering
\caption{Overview of state-of-the-art network architectures considered for model backbone selection. Architectures are compared in terms of parameters and model size, and subdivided into: CNN, Hybrid, Transformer and SSM.}
\begin{tabular}{l | c c}
\toprule
 \textbf{Network architecture} & \textbf{Parameters} & \textbf{Model Size}\\
 & \textbf{(M)} & \textbf{(MB)}\\
\midrule
\textcolor{gray}{\textit{CNN}} & & \\
ResNet-50~\citep{ResNet}                                    & 23.5       &  ~~92.2\\
ConvNeXt-T~\citep{ConvNeXt}                                 & 27.8       & 108.7\\
ConvFormer-S18~\citep{MetaFormerBaselines}                  & 24.7       &  ~~96.7\\
\midrule
\textcolor{gray}{\textit{Hybrid}} & & \\
iFormer-S~\citep{iFormer}                                   & 19.6       &  ~~76.9\\
Uniformer-S+~\citep{UniFormerConference,UniFormerJournal}   & 23.5       &  ~~92.0\\
\hlrev{CAFormer}-S18~\citep{MetaFormerBaselines}                    & 24.3       &  ~~94.9\\
\midrule
\textcolor{gray}{\textit{Transformer}} & & \\
ViT-S/16~\citep{ViT}                                           & 21.7       &  ~~84.8\\
PVTV2-B2~\citep{PvTv2}                                      & 24.9       &  ~~97.2\\
SwinV2-T~\citep{SwinV2}                                     & 27.6       &  109.1\\
\midrule
\textcolor{gray}{\textit{SSM}} & & \\
Vim-S~\citep{ViM}                                           & 25.7       &  100.6\\
\bottomrule
\end{tabular}
\label{table: ExperimentalSetup-SOTA CV Encoders}
\end{table}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Model decoder selection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model decoder selection}
\label{sec: ExperimentalSetup-Decoder}
Several decoders for semantic segmentation are selected for comparison. First, the semantic Feature Pyramid Network (FPN)~\citep{FPN}, which is used as the decoder in the original abstracted MetaFormer approach~\citep{MetaFormerBasic} due to its lightweight and high-performance capabilities in semantic segmentation. FPN employs a simple design to merge information from multiple feature levels of the encoder into a unified output. Another decoder considered is UperNet~\citep{UperNet}, utilized as a decoder in the MetaFormer baselines for vision~\citep{MetaFormerBaselines}, inspired by architectures like ConvNeXt~\citep{ConvNeXtV2} and Swin~\citep{SwinV2}. UperNet addresses the issue of the empirical receptive field of deep CNNs by incorporating a Pyramid Pooling Module on the last layer of the backbone network, which is then fed into a general feature pyramid network. Furthermore, the MobileNetV2 DeepLabV3+ (DLV3+) decoder~\citep{DeepLabV3+,MobileNetV2}, as used in our previous work~\citep{FockensBE2}, leverages atrous convolutions on high-level encoder features, effectively controlling the resolution of computed feature maps prior to merging with low-level features. Lastly, U-Net++~\citep{UNet++} extends the well-established U-Net~\citep{UNet} architecture by redesigning skip pathways with nested and dense skip connections. These connections consist of nested dense convolutional blocks that bridge the semantic gap between encoder and decoder feature maps prior to fusion. A summary and comparison of the considered architectures, including parameters and model size, are provided by Table~\ref{table: ExperimentalSetup-SOTA CV Decoders}. 

%
\begin{table}[t]
\centering
\caption{Overview of state-of-the-art decoders considered for model decoder selection. Architectures are compared in terms of parameters and model size. The selected \hlrev{CAFormer}-S18 backbone is abbreviated as CaF-S18.}
\begin{tabular}{l | c c}
\toprule
 \textbf{Network architecture} & \textbf{Parameters} & \textbf{Model Size}\\
 & \textbf{(M)} & \textbf{(MB)}\\
\midrule
CaF-S18-FPN~\citep{MetaFormerBaselines,FPN}                   & 26.2       &  102.4\\
CaF-S18-UperNet~\citep{MetaFormerBaselines,UperNet}           & 29.5       &  115.4\\
CaF-S18-DLV3+~\citep{MetaFormerBaselines,DeepLabV3+}          & 29.7       &  116.2\\
CaF-S18-U-Net++~\citep{MetaFormerBaselines,UNet++}            & 29.7       &  116.0\\
\bottomrule
\end{tabular}
\label{table: ExperimentalSetup-SOTA CV Decoders}
\end{table}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Training strategies %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training strategies}
\label{sec: ExperimentalSetup-Training}
The process of developing CADe models involves design choices for several training strategies. Each of the considered training strategies, such as domain-specific pre-training, data augmentation techniques, training with additional video frames and segmentation ground-truth utilization, are described in the upcoming subsections.


\subsubsection{Domain-specific pre-training}
\label{sec: ExperimentalSetup-Training-SSL}
Recent innovations in self-supervised learning (SSL) methods, which learn generic representations from unannotated data, have demonstrated that they can outperform supervised pre-training by providing better model initialization~\citep{DINO}. SSL captures a wider variety of features from diverse data, reducing the risk of overfitting to specific labeled datasets and enhancing the model's generalization capabilities. Several studies suggest that using in-domain data for pre-training leads to better performance in downstream tasks~\citep{HeDomainSpecific,PuttenInDomain,ZamirDomainSpecific}. In medical image analysis, the feasibility of SSL methods has been explored~\citep{Ramesh}, and domain-specific self-supervised pre-training has shown superior performance~\citep{SSLXRay,SSLEndoscopy1,SSLPathology,SSLEndoscopy2}. In this study, the selected backbone architecture is pre-trained using in-domain data with an SSL objective. Subsequently, the entire encoder-decoder network is trained for the downstream task. The performance of the resulting model is compared with a variant where the backbone was initialized with standard ImageNet pre-trained weights. The proposed approach enables corroboration of the hypothesis that domain-specific pre-training enhances model performance and robustness, as found in our previous work~\citep{Jaspers-MEDIA,BoersMEDIA}. 

% as found in our previous work --> cite clinical GastroNet

\indent \textsc{A. Dataset}: The GastroNet-5M dataset~\citep{BoersMEDIA} is utilized for in-domain pre-training. This dataset comprises 5,014,174 unlabeled gastrointestinal endoscopic images, collected retrospectively from endoscopic patient databases across 8~Dutch hospitals. For additional details regarding the dataset, we refer to our previous work~\citep{BoersMEDIA}.

% The Gastronet-5M dataset --> cite clinical GastroNet
% we refer to our previous work --> cite clinical GastroNet

\indent \textsc{B. SSL framework}: The well-known SSL objective DINO~\citep{DINO} is employed, which is highly versatile and not restricted to the specific ViT architecture, unlike newer frameworks such as DINOv2~\citep{DINOv2}. DINO uses a teacher-student distillation technique, enabling efficient learning with smaller batch sizes and reducing the need for extensive computational resources. Additionally, DINO updates the weights of the teacher encoder using an exponential moving average (EMA). It eliminates the dependency on negative samples by utilizing a similarity loss, calculated as the cross-entropy loss between the reference positive embeddings. Our implementation closely follows the original, training the selected backbone from scratch. Pre-training is conducted on four 40-GB A100 GPUs (NVIDIA Corp., CA, USA), with a maximum batch size of~544 for 100~epochs. The pre-training stage with GastroNet-5M using the DINO SSL objective is further referred to as \emph{GastroNet} pre-training.
 
\subsubsection{Data augmentation}
\label{sec: ExperimentalSetup-Training-Augmentation}
Data augmentation techniques are applied during training to enhance generalization and virtually increase the dataset size. As described in Section~\ref{sec: MaterialsMethods-Pre-process}, sets of N-DSA and DSA techniques are defined for downstream training. Additionally, corresponding sets of N-DSA and DSA techniques are established for the SSL pre-training stage, described in Section~\ref{sec: ExperimentalSetup-Training-SSL}. Further details regarding the sets of data augmentation techniques can be found in Appendix~\ref{sec: Supplementary-Preprocess}. In our previous work~\citep{Jaspers-MEDIA,RobustnessTool-JaspersAMAI}, these DSA techniques were utilized to generate artificially degraded test sets, simulating clinically calibrated and realistic image degradations, similar to the low-quality endoscopy images often encountered in clinical practice. In this study, the selected encoder-decoder network architecture is pre-trained using the described SSL framework with a specific set of augmentation techniques (N-DSA vs. DSA) each time when the framework is applied. This is followed by downstream training, also utilizing both sets of augmentation techniques. This approach allows to investigate the impact of the data augmentation techniques and their combinations during both pre-training and downstream training, as well as the hypothesis that these augmentation techniques can enhance model performance and robustness when dealing with low-quality imagery. 


\subsubsection{Training with additional video frames}
\label{sec: ExperimentalSetup-Training-VideoFrames}
Videos are available for a subset of prospectively recorded patients, as described in Section~\ref{sec: MaterialsMethods-Data-CADeDatasets}. Key frames are sampled from these videos, based on image quality and semantic information using an in-house tool. The resulting sets of video frames, categorized by defined quality thresholds, are summarized in Table~\ref{table: MaterialsMethods-Data-CADe Datasets}. In this study, the impact is investigated of incorporating additional training frames into the curated training set on the resulting performance. Specifically, the effect is explored of the quantity and quality of the added frames. Experiments are conducted by adding 10\%, 50\% and 100\% of the frames to the curated training set for each set of frames. Additionally, combinations of different quality sets are experimented with, applying the same 10\%, 50\% and 100\% frame-addition strategy. For example, a combination of HQ and MQ frames with 10\% strategy, includes the curated training set supplemented with 10\% of the HQ frames and 10\% of the MQ frames. This approach allows to investigate the hypothesis that incorporating low-quality frames into training enhances model performance and robustness when dealing with low-quality imagery. 

\subsubsection{Segmentation ground-truth utilization}
\label{sec: ExperimentalSetup-Training-GT}
CADe systems focus on the detection (i.e. binary classification and localization) of neoplastic lesions, requiring pixel-level annotations by Barrett's experts. The subtlety of these lesions can lead to significant inter-observer variability among experts, resulting in inconsistent delineation of neoplasia~\citep{BoersCaption}. Often, a fused-consensus ground truth from multiple experts is used~\citep{DeGroof,FockensBE2,Abdelrahim}. However, these binary masks may fail to capture the subtle gradations of neoplasia with a broad range of atypical patterns, crucial for detecting particularly subtle variants. Missing these nuances can prevent the model from accurately identifying the most abnormal tissue for targeted biopsy, leading to disease understaging or missed neoplasia. Several different consensus GT masks with increasing neoplastic certainty can be constructed: Soft-spot GT, Plausible-spot GT, Sweet-spot GT and Hard-spot GT, as described in Section~\ref{sec: MaterialsMethods-Data-CADeDatasets}-E and visualized in Fig.~\ref{fig: MaterialsMethods-Data-GroundTruth}. In addition to these consensus GT masks, various training strategies combining them are established: Random GT, Average GT and Multiple GT, \hlnew{as proposed in our previous work~\citep{Kusters-CaPTion-GTConsensus}}. This study investigates the impact of segmentation ground-truth utilization on the resulting performance. The followed approach allows to investigate how the uncertainty in the data affects the model performance regarding classification, localization and gradual neoplasia coverage of predicted segmentation masks. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Inference strategies %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Inference strategies}
\label{sec: ExperimentalSetup-Inference}
The process of developing CADe models involves design choices for several inference strategies. Each of the considered inference strategies, such as the usage of the model output and TensorRT inference, are described in the upcoming subsections. 


\subsubsection{Usage of the model output}
CADe systems are designed to detect neoplastic lesions through binary classification and localization, typically employing for these tasks either an encoder-decoder architecture~\citep{Ebigbo,DeGroof,FockensBE2,Meinikheim}, or two distinct architectures~\citep{Hussein,Abdelrahim}. Most existing methods in literature follow this approach, where the classification decision is made using the output from either the classification network, or the encoder. However, in our previous work~\citep{FockensBE2} aiming to prioritize a high sensitivity, the maximum pixel value in the segmentation prediction was used as the basis for classification. For the results on the model decoder selection and the training strategies, the performance scores are presented for both the classification branch output and the maximum pixel value from the segmentation prediction. 
However during inference, a single classification decision must be derived from the two outputs, and this study explores the optimal way to combine them for improved performance. Several strategies are considered: using only the classification branch output, using only the maximum pixel value from the segmentation prediction and averaging the two outputs. Additionally, two extra scenarios are defined: (a) either one of the two outputs classification or segmentation output is positive (labeled as OR), and (b) both outputs are positive (labeled as AND). For the average case, the combined average value is used to calculate AUROC and AUPRC scores. In the OR scenario, the highest value of the two outputs determines whether a detection is positive or negative, which is consequently used to compute performance scores. Conversely, in the AND scenario, the lowest value of the two outputs is decisive and therefore used to compute performance scores. The described approach provides a comprehensive analysis of how the outputs from the classification and segmentation branches regarding classification can be optimally combined to maximize classification performance.

 
\subsubsection{TensorRT inference}
Deep learning plays a critical role in developing CADe systems for medical applications, yet the large size and complexity of these networks pose significant challenges, particularly in terms of execution time and demands on computational resources. This discrepancy highlights a gap between the high accuracy achieved in controlled environments and the practical use of these systems in real-world scenarios, where real-time inference on embedded hardware is often required. TensorRT~\citep{TensorRT} addresses this challenge by optimizing inference efficiency without sacrificing accuracy~\citep{ZhouTensorRT}, making it especially valuable for CADe systems that should typically seamlessly integrate with existing medical hardware. Alternatively, when CADe systems are not integrated, they should be easy to use and have limited power consumption and require constrained computational resources.
Unfortunately, many current CADe systems demand substantial computational resources, limiting their utility in real-time video diagnostics and hindering their integration into endoscopy platforms or clinical usage. To mitigate these limitations, our previous work focused on a system specifically designed for direct implementation into existing endoscopy platforms, utilizing a quantized int8-based neural network~\citep{FockensBE2,FockensBE}. Developing this system involved careful consideration of performance-efficiency trade-offs, making the design process complex and intensive. In this study, the impact of the less resource-extensive TensorRT conversion on efficiency and performance is explored. TensorRT is compatible with popular frameworks like PyTorch and Open Neural Network Exchange (ONNX), potentially offering enhanced efficiency without compromising performance. This investigation aims to determine whether TensorRT conversion alone can deliver the desired improvements in efficiency while maintaining the overall system performance.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: SOTA comparison %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{State-of-the-art comparison}
\label{sec: ExperimentalSetup-SOTA}

Numerous studies on Barrett's neoplasia detection have been documented in the literature. In this investigation, the proposed model is benchmarked against a selection of recent deep learning-based approaches designed for Barrett's neoplasia detection. Ebigbo~\textit{et al.}~\citep{Ebigbo} and Meinikheim~\textit{et al.}~\citep{Meinikheim} proposed an encoder-decoder architecture, leveraging ResNet-101 and ResNet-50 encoders, respectively, alongside a DeepLabV3+ decoder. De Groof~\textit{et al.}~\citep{DeGroof} built upon the custom hybrid ResNet-UNet model~\citep{PuttenWLE}. In our replicating experiments, we employ the default ResNet-18 encoder instead of the custom version for utilization of pre-trained weights. Hussein~\textit{et al.}~\citep{Hussein} deployed a ResNet-101 architecture for neoplasia detection and an FCNResNet-50 architecture for neoplasia localization. For our replicating evaluations, the architectures are consolidated into a unified FCNResNet-101 architecture. Similarly, Abdelrahim~\textit{et al.}~\citep{Abdelrahim} followed a comparable strategy, employing a VGG-16-based neoplasia detection model and a SegNet-based localization model. These models are integrated into a single encoder-decoder architecture with a VGG-16 encoder and SegNet decoder for our experiments. Lastly, Fockens~\textit{et al.}~\citep{FockensBE2} introduced a quantized int8-based EfficientNet-lite1 architecture paired with a MobileNetV2-DeepLabV3+ decoder. For all architectures, the backbones are initialized with ImageNet pre-trained weights~\citep{ImageNet}, except for the architecture of Fockens~\textit{et al.}. Since this represents our prior research efforts~\citep{FockensBE2,FockensBE}, we employ the identical network architecture and pre-trained weights from ImageNet + GastroNet in our current implementation. A summary and comparison of the considered architectures from literature, including parameters and model size, are provided by Table~\ref{table: ExperimentalSetup-SOTA BE Detection}.


%
\begin{table}[t]
\centering
\caption{Overview of the state-of-the-art in Barrett's neoplasia detection and the proposed model. Methods are all structured according to the encoder-decoder architecture and are compared in terms of parameters and model size.}
\begin{tabular}{l | c c}
\toprule
 \textbf{Method} & \textbf{Parameters} & \textbf{Model Size}\\
 \textbf{(Encoder-Decoder)} & \textbf{(M)} & \textbf{(MB)}\\
\midrule
Ebigbo \textit{et al.}~\citep{Ebigbo}             &  ~~60.4       & 236.6\\     %241.6
de Groof \textit{et al.}~\citep{DeGroof}          &  ~~13.9       & ~~54.5\\   %~~55.7
Hussein \textit{et al.}~\citep{Hussein}           &  ~~51.9       & 203.5\\     %207.8
Abdelrahim \textit{et al.}~\citep{Abdelrahim}     & 148.9         & 582.0\\     %595.9
Fockens \textit{et al.}~\citep{FockensBE2}        &   ~~~~4.6     & ~~~~5.2\\   %~~~~5.2
Meinikheim \textit{et al.}~\citep{Meinikheim}     &  ~~40.3       & 157.9\\   %161.4
\midrule
Proposed                                          &  ~~29.7       & 116.2\\
\bottomrule
\end{tabular}
\label{table: ExperimentalSetup-SOTA BE Detection}
\end{table}
%


% \subsubsection{Barrett's neoplasia characterization}
% \textcolor{red}{\textbf{
% Numerous studies addresssing Barrett's neoplasia characterization have been published in the literature. In this evaluation, our model is benchmarked against a selection of recent deep learning-based approaches. Struyvenberg~\textit{et al.}~\citep{Struyvenberg} utilized the model proposed by De Groof~\textit{et al.}~\citep{DeGroof} for the classification purpose only, leveraging only the encoder part of the network and implemented in our experiments with a ResNet-18 encoder.  Kusters~\textit{et al.}~\citep{Kusters} devised an EfficientNet-B4 architecture augmented with a custom classification head. Similar to Struyvenberg~\textit{et al.}'s approach, the works of Hussein~\textit{et al.}~\citep{HusseinCADx} and Jukema~\textit{et al.}~\citep{Jukema} are based on their respective Barrett's neoplasia detection frameworks. Hussein~\textit{et al.} exclusively employs the ResNet-101 architecture for classification objectives, while Jukema~\textit{et al.} utilizes the quantized int8-based EfficientNet-lite1 component from the architecture proposed by Fockens \textit{et al.}~\citep{FockensBE2}. Given that the efforts of Kusters~\textit{et al.} and Jukema~\textit{et al.} are derived from our prior research efforts, we maintain consistency by employing the identical network architecture and ImageNet + GastroNet pre-trained weights in our current implementation. Conversely, for other methodologies, ImageNet-pre-trained weights are utilized and our own implementation is adopted, as explained for the neoplasia detection models. A summary and comparison of the considered architectures from literature, including parameters and model size, are provided in Table~\ref{table: ExperimentalSetup-SOTA BE Characterization}.}}


% %
% \begin{table}[t]
% \centering
% \caption{Overview of the state-of-the-art in Barrett's neoplasia characterization and our model. Methods are compared in terms of parameters and model size. \textcolor{red}{\textbf{Replace Model Size (MB) with actual size of final pytorch model!!}}}
% \begin{tabular}{l | c c}
% \toprule
%  \textbf{Method} & \textbf{Parameters} & \textbf{Model Size}\\
%   & \textbf{(M)} & \textbf{(MB)}\\
% \midrule
% Struyvenberg \textit{et al.}~\citep{Struyvenberg} &  11.6       & ~~46.3\\
% Kusters \textit{et al.}~\citep{Kusters}           &  20.4       & ~~12.1\\
% Hussein \textit{et al.}~\citep{HusseinCADx}       &  42.5       & 170.0\\
% Jukema \textit{et al.}~\citep{Jukema}             &   ~~4.2     &  ~~~~4.8\\
% \midrule
% Ours                                              &               & \\
% \bottomrule
% \end{tabular}
% \label{table: ExperimentalSetup-SOTA BE Characterization}
% \end{table}
% %

==> Sections/5-ResultsDiscussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RESULTS & DISCUSSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section presents and discusses the outcomes of the experiments conducted to evaluate the design choices for the structured development of CADe systems for Barrett's neoplasia detection, as summarized in Section~\ref{sec: ExperimentalSetup} and Fig.\ref{fig: ExperimentalSetup}. The results and discussion on backbone selection are detailed in Section~\ref{sec: ResultsDiscussion-Backbone}, followed by the selection of the semantic segmentation decoder in Section~\ref{sec: ResultsDiscussion-Decoder}. The discussion of the results follows exactly the same order and numbering as described in the setup (Section~\ref{sec: ExperimentalSetup}). Hence, Section~\ref{sec: ResultsDiscussion-Training} focuses on the results from various training strategies, while Section~\ref{sec: ResultsDiscussion-Inference} addresses the outcomes of different inference strategies. Finally, Section~\ref{sec: ResultsDiscussion-SOTA} presents the benchmarking results of the proposed approach against state-of-the-art Barrett's neoplasia detection algorithms.

%
\begin{table*}[t]
    \centering
        \caption{Classification performances of all backbones on the validation sets. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}
        \begin{tabular}{ l | c c c c c c}
             \toprule
              \textbf{Backbone} &\multicolumn{2}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-3}
             \cmidrule(lr){4-5}
             \cmidrule(lr){6-7}
             & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ \\
             \midrule
             \textcolor{gray}{\textit{CNN}} &  &  &  &  &  &  \\
             ResNet-50~\citep{ResNet}                       & 0.942\sd{.005} & 0.938\sd{.010} & 0.938\sd{.004} & 0.941\sd{.004} & \textbf{0.875\sd{.016}} & \textbf{0.862\sd{.019}} \\
             ConvNeXt-T~\citep{ConvNeXt}                    & 0.943\sd{.011} & 0.940\sd{.012} & 0.918\sd{.011} & 0.927\sd{.010} & 0.861\sd{.039} & 0.824\sd{.031} \\
             ConvFormer-S18~\citep{MetaFormerBaselines}     & 0.942\sd{.015} & 0.938\sd{.014} & 0.925\sd{.015} & 0.934\sd{.012} & 0.847\sd{.023} & 0.819\sd{.026} \\
             \midrule
             \textcolor{gray}{\textit{Hybrid}} &  &  &  &  &  &  \\
             iFormer-S~\citep{iFormer}                                  & 0.943\sd{.035} & 0.937\sd{.035} & 0.928\sd{.031} & 0.928\sd{.028} & 0.852\sd{.042} & 0.828\sd{.045} \\
             UniFormer-S+~\citep{UniFormerConference,UniFormerJournal}  & 0.959\sd{.004} & 0.957\sd{.003} & 0.939\sd{.005} & \textbf{0.947\sd{.004}} & 0.870\sd{.012} & 0.847\sd{.018} \\
             \hlrev{CAFormer}-S18~\citep{MetaFormerBaselines}                   & \textbf{0.961\sd{.002}} & \textbf{0.958\sd{.002}} & \textbf{0.941\sd{.006}} & \textbf{0.947\sd{.006}} & 0.856\sd{.016} & 0.841\sd{.017} \\
             \midrule
             \textcolor{gray}{\textit{Transformer}} &  &  &  &  &  &  \\
             ViT-S/16~\citep{ViT}                           & 0.919\sd{.017} & 0.918\sd{.019} & 0.904\sd{.021} & 0.913\sd{.021} & 0.833\sd{.029} & 0.814\sd{.031} \\
             PVTv2-B2~\citep{PvTv2}                         & 0.940\sd{.017} & 0.936\sd{.020} & 0.927\sd{.013} & 0.933\sd{.011} & 0.817\sd{.027} & 0.798\sd{.031} \\
             SwinV2-T~\citep{SwinV2}                        & 0.951\sd{.019} & 0.949\sd{.021} & 0.939\sd{.011} & 0.945\sd{.011} & 0.858\sd{.010} & 0.831\sd{.012} \\
             \midrule
             \textcolor{gray}{\textit{SSM}} &  &  &  &  &  &  \\
             Vim-S~\citep{ViM}                              & 0.954\sd{.005} & 0.951\sd{.005} & \textbf{0.941\sd{.009}} & 0.945\sd{.008} & 0.859\sd{.024} & 0.849\sd{.022} \\
            \bottomrule  
        \end{tabular}
    \label{table: ResultsDiscussion-Backbone}
\end{table*}
%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Backbone selection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model backbone selection - evaluation}
\label{sec: ResultsDiscussion-Backbone}
The classification performance results of the compared backbone architectures on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Backbone}. For the design of the CADe framework, the \hlrev{CAFormer}-S18 architecture has been selected as the backbone. This decision is primarily based on the performance on the Images+HQ Frames and MQ Frames validation sets. Although its performance on the LQ Frames validation set is relatively limited, this is less critical in practical applications, since CADe systems are envisioned to be integrated with Computer-Aided Quality (CAQ) systems. These CAQ systems assess frame informativeness~\citep{PuttenFIA,MammadliFIA}, ensuring that only frames with sufficient quality are provided to the CADe system, thereby reducing the impact of severe low-quality frames on the detection performance. Additionally, as shown in Table~\ref{table: ExperimentalSetup-SOTA CV Encoders}, the comparison of parameters and model size places \hlrev{CAFormer}-S18 in the middle range among the architectures considered. The final decision between \hlrev{CAFormer}-S18 and UniFormer-S+ is influenced by \hlrev{CAFormer}-S18's status as a newer and more versatile architecture, providing a more generic solution compared to UniFormer-S+. The reader should notice that the two best-performing models have a hybrid CNN-Transformer architecture, which enables the optimal learning and exploitation of the strengths of both network designs. 

% The classification performance results of the compared backbone architectures on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Backbone}. For the Images+HQ Frames validation set, CAFormer-S18 achieves the best performance in both AUROC$_{cls}$ and AUPRC$_{cls}$, with narrow margins of 0.1\% and 0.2\%, respectively. The only backbone that approaches the performance of CAFormer-S18 is UniFormer-S+. A similar trend is observed for the MQ Frames validation set. However, the best performance is shared among CAFormer-S18, Vim-S, and UniFormer-S+, depending on the specific metric of AUROC$_{cls}$ and AUPRC$_{cls}$, respectively. For the LQ Frames validation set, ResNet-50 achieves the highest scores for both classification metrics, with margins of 0.5\% and 1.3\% for AUROC$_{cls}$ and AUPRC$_{cls}$, respectively.
% For the design of the CADe framework, the CAFormer-S18 architecture has been selected as the backbone. This decision is primarily based on the performance on the Images+HQ Frames and MQ Frames validation sets. Although its performance on the LQ Frames validation set is relatively limited, this is less critical in practical applications, as CADe systems are envisioned to be integrated with Computer-Aided Quality (CAQ) systems. These CAQ systems assess frame informativeness~\citep{PuttenFIA,MammadliFIA}, ensuring that only frames with sufficient quality are provided to the CADe system, thereby reducing the impact of extremely low-quality frames on the detection performance. Additionally, a comparison of parameters and model size, as shown in Table~\ref{table: ExperimentalSetup-SOTA CV Encoders}, places CAFormer-S18 in the middle range among the architectures considered. The final decision between CAFormer-S18 and UniFormer-S+ was influenced by CAFormer-S18's status as a newer and more versatile architecture, providing a more generic solution compared to UniFormer-S+.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Decoder selection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model decoder selection - evaluation}
\label{sec: ResultsDiscussion-Decoder}
The classification, classification-by-segmentation and localization performance results of the selected \hlrev{CAFormer}-S18 backbone in combination with the considered decoder architectures, on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Decoder}. It can be observed from the obtained results that the DeepLabV3+ and FPN decoders perform very similar in terms of classification performance across all three validation sets, while DeepLabV3+ achieves the best results for almost every metric in the classification-by-segmentation task, especially in the MQ and LQ Frames sets. Although U-Net++ significantly outperforms other architectures in the localization task, it underperforms compared to DeepLabV3+ and FPN across other metrics. Good localization performance with lower classification-by-segmentation scores is suboptimal, because a good Dice score for the segmentation does not ensure correct classification+localization. The classification-by-segmentation score indicates only whether segmentation masks are incorrectly produced for negative cases or missed for positive cases. Therefore, a high classification-by-segmentation score is essential, as the CADe system should function as a detection algorithm, where near-perfect segmentation is less important and flagging suspicious tissue is more important. Consequently, the DeepLabV3+ decoder architecture is selected for the design of the CADe algorithm, since it consistently achieves the best performance for the classification-by-segmentation metrics across all validation sets. Additionally, despite having the largest number of parameters and model size, the superior performance of the selected architecture justifies these factors, as the differences in parameter count and model size are marginal.

% The classification, classification-by-segmentation and localization performance results of the selected CAFormer-S18 backbone in combination with considered decoder architectures on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Decoder}. For the performance on the Images+HQ Frames validation set, the network architectures incorporating DeepLabV3+ and FPN decoders share the top scores in AUROC$_{cls}$, AUPRC$_{cls}$ and AUPRC$_{seg}$. The DeepLabV3+ architecture also achieves the best performance in AUROC$_{seg}$ with a margin of 0.5\%, while the U-Net++ architecture excels in localization performance, as measured by $mD_i$, with a margin of 3.6\%. Similar trends are observed in the MQ Frames validation set, where DeepLabV3+ and FPN decoders achieve equal scores in AUROC$_{cls}$, and FPN leads in AUPRC$_{cls}$ with a margin of 0.1\%. However, DeepLabV3+ surpasses other decoders in AUROC$_{seg}$ and AUPRC$_{seg}$, with margins of 1.4\% and 0.5\%, respectively. In the LQ Frames validation set, the DeepLabV3+ architecture consistently outperforms others in AUROC$_{cls}$, AUROC$_{seg}$ and AUPRC$_{seg}$, with margins of 0.7\%, 1.8\% and 0.3\%, respectively. Conversely, the FPN architecture achieves the highest performance in AUPRC$_{cls}$ with a margin of 2.0\%. 
% As is evident from the obtained results, the DeepLabV3+ and FPN decoders perform very similar in terms of classification performance, while DeepLabV3+ achieves the best results for almost every metric in the classification-by-segmentation task. Although U-Net++ significantly outperforms other architectures in the localization task, it underperforms compared to DeepLabV3+ and FPN across other metrics. Good localization performance with lower classification-by-segmentation scores is suboptimal, as the classification-by-segmentation score indicates whether segmentations are incorrectly produced for negative cases or missed for positive cases, even if a good Dice score is achieved on actually segmented positive cases. Therefore, a higher classification-by-segmentation score is preferred, as the CADe system should function as a detection algorithm, where near-perfect segmentations are less crucial and flagging suspicious tissue is more important. Consequently, the DeepLabV3+ decoder architecture is selected for the design of the CADe algorithm, as it consistently achieves the best performance for the classification-by-segmentation metrics across all validation sets. Additionally, despite having the largest number of parameters and model size, the selected architecture's superior performance justifies these factors, as the differences in parameter count and model size are marginal.

%
\begin{table*}[t]
    \centering
        \caption{Classification, classification-by-segmentation and localization performance of the selected \hlrev{CAFormer}-S18 backbone in combination with considered decoders on the different validation sets. $mD_i$ stands for Dice score in segmentation. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}
        \begin{tabular}{ l | c c c c c c c}
             \toprule
              \textbf{Decoder} &\multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{cls}$ & AUPRC$_{cls}$ & $mD_i$ & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ \\
             \midrule
             FPN~\citep{FPN}                & \textbf{0.958\sd{.011}} & \textbf{0.956\sd{.011}} & 0.558\sd{.035} & \textbf{0.937\sd{.012}} & \textbf{0.945\sd{.009}} & 0.827\sd{.016} & \textbf{0.836\sd{.046}}\\
             UperNet~\citep{UperNet}        & 0.946\sd{.026} & 0.943\sd{.027} & 0.496\sd{.146} & 0.927\sd{.018} & 0.934\sd{.019} & 0.823\sd{.019} & 0.803\sd{.034}\\
             DeepLabV3+~\citep{DeepLabV3+}  & \textbf{0.958\sd{.007}} & \textbf{0.956\sd{.008}} & 0.544\sd{.012} & \textbf{0.937\sd{.009}} & 0.944\sd{.006} & \textbf{0.834\sd{.025}} & 0.816\sd{.020}\\
             U-Net++~\citep{UNet++}         & 0.955\sd{.001} & 0.953\sd{.003} & \textbf{0.596\sd{.030}} & 0.933\sd{.002} & 0.941\sd{.003} & 0.826\sd{.022} & 0.811\sd{.011}\\
            \midrule
            \midrule
             \textbf{Decoder} & \multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{seg}$ & AUPRC$_{seg}$ & & AUROC$_{seg}$ & AUPRC$_{seg}$ & AUROC$_{seg}$ & AUPRC$_{seg}$ \\
             \midrule
             FPN~\citep{FPN}                & 0.950\sd{.010} & \textbf{0.952\sd{.009}} &  & 0.918\sd{.010} & 0.935\sd{.007} & 0.774\sd{.028} & 0.781\sd{.022}\\
             UperNet~\citep{UperNet}        & 0.936\sd{.015} & 0.937\sd{.020} & & 0.908\sd{.015} & 0.922\sd{.019} & 0.804\sd{.020} & 0.790\sd{.038}\\
             DeepLabV3+~\citep{DeepLabV3+}  & \textbf{0.955\sd{.008}} & \textbf{0.952\sd{.010}} & & \textbf{0.932\sd{.012}} & \textbf{0.940\sd{.009}} & \textbf{0.822\sd{.020}} & \textbf{0.793\sd{.013}}\\
             U-Net++~\citep{UNet++}         & 0.945\sd{.008} & 0.946\sd{.006} & & 0.917\sd{.011} & 0.930\sd{.007} & 0.796\sd{.028} & 0.787\sd{.021}\\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-Decoder}
\end{table*}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Training strategies %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training strategies}
\label{sec: ResultsDiscussion-Training}
This subsection presents and discusses the outcomes of the experiments conducted to evaluate the design choices regarding various training strategies, such as domain-specific pre-training, data augmentation techniques, training with additional video frames and segmentation ground-truth utilization, in Section~\ref{sec: ResultsDiscussion-Training-SSL}, \ref{sec: ResultsDiscussion-Training-Augmentation}, \ref{sec: ResultsDiscussion-Training-VideoFrames} and \ref{sec: ResultsDiscussion-Training-GT}, respectively.


\subsubsection{Domain-specific pre-training - evaluation}
\label{sec: ResultsDiscussion-Training-SSL}
The classification, classification-by-segmentation and localization performance results of the optimal network architecture with ImageNet and GastroNet pre-training, on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Training-SSL}. As is immediately clear, across all metrics and validation sets, the GastroNet pre-training significantly outperforms the ImageNet pre-trained counterpart, especially for the MQ Frames and LQ Frames validation sets with pronounced improvements up to 7.8\%. From these observations, it can be concluded that GastroNet pre-training is superior to ImageNet pre-training, confirming the hypothesis that an SSL pre-training objective combined with an in-domain dataset indeed captures a wider variety of features and enhances the model's generalization capabilities and robustness against low-quality data. This finding is fully in line with our previous research efforts~\citep{Jaspers-MEDIA,BoersMEDIA}. Therefore, GastroNet pre-training is selected as the pre-training strategy for the design of the CADe algorithm.

% The classification, classification-by-segmentation and localization performance results of the optimal network architecture with ImageNet and GastroNet pre-training on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Training-SSL}. As is immediately obvious, across all metrics and validation sets, the GastroNet pre-training significantly outperforms the ImageNet pre-trained counterpart. More specifically, for the Images+HQ Frames validation set GastroNet pre-training improves upon ImageNet pre-training by 1.6\%, 1.7\%, 2.0\%, 2.2\% and 7.3\% for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$, AUPRC$_{seg}$ and $mD_i$, respectively. Similar trends are observed for the MQ Frames validation set, with improvements of 2.5\%, 2.4\%, 2.9\% and 2.4\%, for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$ and AUPRC$_{seg}$, respectively. For the LQ Frames validation set, the improvements are even more pronounced, with increases of 5.5\%, 6.8\%, 5.7\% and 7.8\%, for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$ and AUPRC$_{seg}$, respectively. From these observations, it can be concluded that GastroNet pre-training is superior to ImageNet pre-training, especially for the lower-quality validation sets, confirming the hypothesis that an SSL pre-training objective combined with an in-domain dataset indeed captures a wider variety of features and enhances the model's generalization capabilities and robustness against lower-quality data, in line with our previous research efforts~\citep{Jaspers-MEDIA,BoersMEDIA}. Therefore, GastroNet pre-training is selected as the pre-training strategy for the design of the CADe algorithm. 

%
\begin{table*}[t]
    \centering
        \caption{Classification, classification-by-segmentation and localization performance of the optimal network architecture with considered pre-training strategies, on the different validation sets. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}
        \begin{tabular}{ l | c c c c c c c}
             \toprule
              \textbf{Pre-training} &\multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{cls}$ & AUPRC$_{cls}$ & $mD_i$ & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ \\
             \midrule
             ImageNet         & 0.958\sd{.007} & 0.956\sd{.008} & 0.544\sd{.012} & 0.937\sd{.009} & 0.944\sd{.006} & 0.834\sd{.025} & 0.816\sd{.020}\\
             GastroNet        & \textbf{0.974\sd{.004}} & \textbf{0.973\sd{.003}} & \textbf{0.617\sd{.017}} & \textbf{0.962\sd{.003}} & \textbf{0.968\sd{.003}} & \textbf{0.889\sd{.014}} & \textbf{0.884\sd{.013}}\\
            \midrule
            \midrule
             \textbf{Pre-training} & \multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{seg}$ & AUPRC$_{seg}$ & & AUROC$_{seg}$ & AUPRC$_{seg}$ & AUROC$_{seg}$ & AUPRC$_{seg}$ \\
             \midrule
             ImageNet         & 0.955\sd{.008} & 0.952\sd{.010} & & 0.932\sd{.012} & 0.940\sd{.009} & 0.822\sd{.020} & 0.793\sd{.013}\\
             GastroNet        & \textbf{0.975\sd{.003}} & \textbf{0.974\sd{.004}} & & \textbf{0.961\sd{.004}} & \textbf{0.964\sd{.004}} & \textbf{0.879\sd{.011}} & \textbf{0.871\sd{.011}} \\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-Training-SSL}
\end{table*}
%

\subsubsection{Data augmentation - evaluation}
\label{sec: ResultsDiscussion-Training-Augmentation}
The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with the considered data augmentation strategies, on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Training-Augmentation}. It is evident from the obtained results, that employing DSA techniques in either the pre-training or downstream training stage leads to detrimental performance on the Images+HQ Frames validation set. In contrast, employing DSA techniques in one of the two stages often improves performance on the MQ Frames and LQ Frames validation sets compared to using default techniques in both stages. However, when DSA techniques are applied in both stages, it clearly results in poorer performance. This detrimental performance may be explained by the fact that DSA techniques involve more simultaneously applied transformations, which can confuse model training rather than having benefit from it. Another possible explanation is that the operating ranges of the DSA techniques are smaller, potentially reducing their effectiveness. The increased performance on low-quality images confirms the hypothesis that DSA effectively simulates real-world issues like blur and overexposure, as seen in the low-quality validation sets. Although employing N-DSA in pre-training and DSA in downstream training demonstrates increased robustness on low-quality validation sets, it compromises performance on clean images. Therefore, N-DSA techniques are selected for both pre-training and downstream training in the CADe design. This approach prioritizes performance on clean images, even if it results in slightly reduced robustness on low-quality data, which is favored by clinicians and connects with the envisioned integration into CAQ systems in clinical practice.

% The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with the considered data augmentation strategies on the three validation sets are presented in Table~\ref{table: ResultsDiscussion-Training-Augmentation}. For the performance on the Images+HQ Frames validation set, utilizing N-DSA in both pre-training and downstream training achieves the best performance with margins of 0.2\%, 0.1\%, 0.6\%, 0.5\% and 1.2\% for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$, AUPRC$_{seg}$ and $mD_i$, respectively. This trend is similarly observed for the MQ Frames validation set, where employing N-DSA in both pre-training and downstream training results in the best performance for AUPRC$_{cls}$ with a margin of 0.1\%, while for AUROC$_{cls}$ it matches the performance of the combination of DSA in pre-training and N-DSA in downstream training. For AUROC$_{seg}$ and AUPRC$_{seg}$, the combination of DSA in pre-training and N-DSA in downstream training achieves the best score with margins of 0.2\% and 0.3\%, respectively. For the LQ Frames validation set, the combination of N-DSA in pre-training and DSA in downstream training yields the best performance with margins of 0.7\%, 0.8\%, 1.5\% and 0.7\% for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$ and AUPRC$_{seg}$ respectively. What is evident from the obtained results, is that employing DSA techniques in either the pre-training or downstream training stage leads to detrimental performance on the high-quality validation set. In contrast, employing DSA techniques in one of the two stages often improves performance on the lower-quality validation set compared to using default techniques in both stages. However, when DSA techniques are applied in both stages, it clearly results in poorer performance. This detrimental performance may be explained by the fact that DSA techniques involve more simultaneously applied transformations, which can confuse model training rather than having benefit from it. Another possible explanation is that the operating ranges of the DSA techniques are narrower, potentially reducing their effectiveness. The increased performance on lower-quality images confirms the hypothesis that DSA effectively simulates real-world issues like blur and overexposure, as seen in the lower-quality validation sets. Although employing N-DSA in pre-training and DSA in downstream training demonstrates increased robustness on lower-quality validation sets, it compromises performance on clean images. Therefore, N-DSA techniques are selected for both pre-training and downstream training in the CADe design. This approach prioritizes performance on clean images, even if it results in slightly reduced robustness on lower-quality data. 

%
\begin{table*}[t]
    \centering
        \caption{Classification, classification-by-segmentation and localization performance of the optimal network architecture using previously selected training design choices considered data augmentation strategies, on the different validation sets. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface. The first column describes the set of augmentation techniques employed in the SSL pre-training stage and downstream training (i.e. pre-training - downstream).}
        \begin{tabular}{ l | c c c c c c c}
             \toprule
              \textbf{Augmentation} &\multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             \textbf{(Pre-training - downstr.)}& AUROC$_{cls}$ & AUPRC$_{cls}$ & $mD_i$ & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ \\
             \midrule
             N-DSA - N-DSA        & \textbf{0.974\sd{.004}} & \textbf{0.973\sd{.003}} & \textbf{0.617\sd{.017}} & \textbf{0.962\sd{.003}} & \textbf{0.968\sd{.003}} & 0.889\sd{.014} & 0.884\sd{.013}\\
             N-DSA - DSA         & 0.965\sd{.001} & 0.966\sd{.001} & 0.596\sd{.012} & 0.955\sd{.004} & 0.963\sd{.002} & \textbf{0.896\sd{.011}} & \textbf{0.892\sd{.010}}\\
             DSA - N-DSA         & 0.972\sd{.005} & 0.972\sd{.004} & 0.605\sd{.020} & \textbf{0.962\sd{.006}} & 0.967\sd{.005} & 0.885\sd{.015} & 0.882\sd{.012}\\
             DSA - DSA          & 0.969\sd{.007} & 0.969\sd{.006} & 0.603\sd{.025} & 0.955\sd{.008} & 0.962\sd{.006} & 0.882\sd{.027} & 0.876\sd{.023}\\
            \midrule
            \midrule
             \textbf{Augmentation} & \multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             \textbf{(Pre-training - downstr.)} & AUROC$_{seg}$ & AUPRC$_{seg}$ & & AUROC$_{seg}$ & AUPRC$_{seg}$ & AUROC$_{seg}$ & AUPRC$_{seg}$ \\
             \midrule
             N-DSA - N-DSA        & \textbf{0.975\sd{.003}} & \textbf{0.974\sd{.004}} & & 0.961\sd{.004} & 0.964\sd{.004} & 0.879\sd{.011} & 0.871\sd{.011} \\
             N-DSA - DSA         & 0.967\sd{.005} & 0.966\sd{.005} & & 0.959\sd{.003} & 0.961\sd{.003} & \textbf{0.896\sd{.014}} & \textbf{0.882\sd{.010}}\\
             DSA - N-DSA         & 0.969\sd{.004} & 0.969\sd{.004} & & \textbf{0.963\sd{.004}} & \textbf{0.967\sd{.004}} & 0.876\sd{.041} & 0.876\sd{.025}\\
             DSA - DSA          & 0.967\sd{.003} & 0.966\sd{.004} & & 0.958\sd{.005} & 0.963\sd{.004} & 0.881\sd{.036} & 0.875\sd{.026}\\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-Training-Augmentation}
\end{table*}
%

\subsubsection{Training with additional video frames - evaluation}
\label{sec: ResultsDiscussion-Training-VideoFrames}
The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with considered video frame addition strategies, on the three validation sets are displayed in Table~\ref{table: Supplementary-VideoFrames} and presented in Appendix~\ref{sec: Supplementary-VideoFrames}. Furthermore, visually informative bar plots, summarizing the performance are depicted in Fig.~\ref{fig: ResultsDiscussion-Training-VideoFrames}. From Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUPRCSEG}, it is evident that on the clean Images+HQ Frames validation set, the performance without additional frames is either the best or only marginally worse than the best experiment. For localization, several experiments surpass the reference experiment, which is particularly interesting, considering that the additional frames are not accompanied with additional segmentation masks for training. From Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUPRCSEG}, for the MQ Frames validation set, more experiments with additional video frames outperform the reference performance, particularly in classification-by-segmentation. Similar observations are clear for the LQ Frames validation set in Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUPRCSEG}, where for classification performance, only one or two experiments surpass the reference performance, whereas in classification-by-segmentation, almost all experiments exceed the reference performance. These observations confirm the hypothesis that incorporating low-quality frames during training may slightly reduce performance on clean images but significantly enhances the model robustness against low-quality images. The reader may expect that incorporating especially HQ Frames would enhance performance on clean images by increasing the dataset size. However, because the video frames originate from a limited patient pool, the diversity of the additional frames is restricted, which constrains potential performance improvements. Ideally, to fully assess the impact on model performance, this scenario would be tested using video frames from all patients in the training set, rather than just a subset. For the design of the CADe system, the strategy of adding 10\% HQ-MQ frames is selected, as the performance difference on clean images is negligible, while providing a higher performance compared to the reference performance on the low-quality sets.

% The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with considered video frame addition strategies on the three validation sets are displayed in Table~\ref{table: Supplementary-VideoFrames} presented in Appendix~\ref{sec: Supplementary-VideoFrames}. Furthermore, visually informative bar plots, summarizing the performance are depicted in Fig.~\ref{fig: ResultsDiscussion-Training-VideoFrames}. 

% For the performance on the Images+HQ Frames validation set, visualized in Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUPRCSEG}, the reference experiment without additional frames achieves the best performance for AUROC$_{cls}$ and AUPRC$_{cls}$, with margins of 0.1\% for both metrics. For AUROC$_{seg}$ and AUPRC$_{seg}$, the reference performance is only 0.1\% below the best performance. Regarding the localization performance, the addition of 10\% MQ-LQ yields the highest performance, with a margin of 0.8\% over the second-best performance and 2.3\% over the reference performance. For the performance on the MQ Frames validation set, visualized in Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUPRCSEG}, the experiment with 10\% HQ-MQ achieves the highest scores for AUROC$_{cls}$ and AUPRC$_{cls}$, with margins of 0.1\% for both metrics over the second-best performance, which is the reference experiment without additional frames. Similarly, for AUROC$_{seg}$ and AUPRC$_{seg}$, the experiment with 10\% HQ-MQ again secures the top performance, with margins of 0.2\% and 0.1\% over the second-best performance and 0.5\% and 0.4\% over the reference performance without additional frames. For the performance on the LQ Frames validation set, visualized in Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUPRCSEG}, the 10\% HQ-MQ strategy continues to achieve the best results for AUROC$_{cls}$ and AUPRC$_{cls}$, with margins of 0.4\% and 0.2\% over the second-best performance and 0.4\% for both metrics over the reference performance, respectively. For AUROC$_{seg}$ and AUPRC$_{seg}$, the experiment with 50\% LQ additional frames emerges as the top performer, with margins of 0.3\% and 0.1\% over the second-best and 2.0\% and 1.9\% over the reference performance, respectively. 

% From Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-HQAUPRCSEG}, it is evident that on the clean Images+HQ Frames validation set, the performance without additional frames is either the best or only marginally worse than in one or two other experiments. For localization, several experiments surpass the reference experiment, which is particularly interesting considering that the additional frames are not accompanied with additional segmentation masks for training. From Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-MQAUPRCSEG}, for the MQ Frames validation set, more experiments with additional video frames outperform the reference performance, particularly in classification-by-segmentation. Similar observations are evident for the LQ Frames validation set in Figs.~\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUROCCLS}-\ref{fig: ResultsDiscussion-Training-VideoFrames-LQAUPRCSEG}, where for classification performance, only one or two experiments surpass the reference performance, whereas in classification-by-segmentation, almost all experiments exceed the reference performance. These observations confirm the hypothesis that incorporating lower-quality frames during training may slightly reduce performance on clean images but significantly enhances the model's robustness against lower-quality images. One might anticipate that incorporating especially HQ Frames would enhance performance on clean images by increasing the dataset size. However, because the video frames originate from a limited patient pool, the diversity of the additional frames is restricted, which constrains potential performance improvements. Ideally, this scenario would be tested using video frames from all patients in the training set, rather than just a subset, to fully assess the impact on model performance. For the design of the CADe system, the strategy of adding 10\% HQ-MQ frames is selected, as it only marginally underperforms on the clean images, while outperforming the reference performance the lower-quality sets. 


%
\begin{figure*}[t!]
\centering

    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/Images + HQ Frames_AUROC_CLS.pdf }
        \caption{Images + HQ Frames: AUROC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-HQAUROCCLS}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/Images + HQ Frames_AUPRC_CLS.pdf }
        \caption{Images + HQ Frames: AUPRC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-HQAUPRCCLS}
    \end{subfigure}%
        \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/Images + HQ Frames_Dice.pdf}
        \caption{Images + HQ Frames: $mD_i$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-HQDICE}
    \end{subfigure}%
    \hspace{\fill}

    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/Images + HQ Frames_AUROC_SEG.pdf }
        \caption{Images + HQ Frames: AUROC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-HQAUROCSEG}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/Images + HQ Frames_AUPRC_SEG.pdf }
        \caption{Images + HQ Frames: AUPRC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-HQAUPRCSEG}
    \end{subfigure}%
    \hspace{\fill}

    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/MQ Frames_AUROC_CLS.pdf }
        \caption{MQ Frames: AUROC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-MQAUROCCLS}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/MQ Frames_AUPRC_CLS.pdf }
        \caption{MQ Frames: AUPRC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-MQAUPRCCLS}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/MQ Frames_AUROC_SEG.pdf }
        \caption{MQ Frames: AUROC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-MQAUROCSEG}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/MQ Frames_AUPRC_SEG.pdf }
        \caption{MQ Frames: AUPRC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-MQAUPRCSEG}
    \end{subfigure}%


    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/LQ Frames_AUROC_CLS.pdf }
        \caption{LQ Frames: AUROC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-LQAUROCCLS}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/LQ Frames_AUPRC_CLS.pdf }
        \caption{LQ Frames: AUPRC$_{cls}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-LQAUPRCCLS}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/LQ Frames_AUROC_SEG.pdf }
        \caption{LQ Frames: AUROC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-LQAUROCSEG}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figures/Video Frames/LQ Frames_AUPRC_SEG.pdf }
        \caption{LQ Frames: AUPRC$_{seg}$}
        \label{fig: ResultsDiscussion-Training-VideoFrames-LQAUPRCSEG}
    \end{subfigure}%

    \caption{Bar plots indicating the performance of the reference experiments without additional frames and all the experiments with frame addition strategies for all metrics and validation sets. The dashed line for reference performance is supplemented with an error band indicating the standard deviation of the experiments, while bar plots are supplemented with vertical error bars indicating the standard deviation of the experiments. }
    \label{fig: ResultsDiscussion-Training-VideoFrames}
\end{figure*}
%




\subsubsection{Segmentation ground-truth utilization - evaluation}
\label{sec: ResultsDiscussion-Training-GT}
The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with considered segmentation ground-truth utilization, on the three validation sets are displayed in Table~\ref{table: ResultsDiscussion-Training-GT}. Furthermore, example lesions with corresponding Average GT and predicted segmentation masks of all the considered models are depicted in Fig.~\ref{fig: ResultsDiscussion-Training-GT}. The results clearly demonstrate a decline in performance across all validation sets, when transitioning from the model trained with Soft-spot GT to the counterpart trained with Hard-spot GT strategy. This decline is particularly pronounced in localization performance, as measured by $mD_i$, which shows a significant drop. This reduction in performance is due to the evaluation process relying on the default Plausible-spot GT, which does not align with the smaller, more focused Hard-spot GT strategy used during training. Furthermore, as illustrated in Columns~3-6 of Fig.~\ref{fig: ResultsDiscussion-Training-GT}, there is a clear decrease in the size of the predicted segmentation masks, as the strategy shifts from Soft-spot GT to Hard-spot GT. This pattern reflects the differences in the training data, where the segmentation GT masks used in training vary in size and neoplastic certainty, which is also illustrated in Fig.~\ref{fig: MaterialsMethods-Data-GroundTruth}. The Soft-spot GT training strategy leads to large predicted masks with high confidence, capturing atypical and neoplastic areas with equal intensity. In contrast, the Hard-spot GT training strategy results in highly condensed masks that focus primarily on the regions deemed most neoplastic during training. These findings suggest that training with masks that prioritize higher neoplastic certainty may inadvertently lead to the omission of subtle lesions, or subtle parts of larger lesions, thereby producing smaller predicted masks which ultimately deteriorate the detection performance.

Further interesting patterns emerge in Columns~7-9 of Fig.~\ref{fig: ResultsDiscussion-Training-GT}. By the nature of the Random GT training strategy, the model is forced to learn a generalized form of all consensus GT masks. This is evident in the predicted masks, since they are an intermediate form of the predicted masks of the Plausible-spot GT and Sweet-spot GT trained models. Both the Multiple GT and Average GT strategies expose the model to all consensus GT masks during training, but they lead to different outcomes. The Average GT approach results in segmentation masks with lower confidence, likely due to the non-binary nature causing predictions to be non-binary. In contrast, the Multiple GT strategy compels the model to generalize across all consensus GT masks, but with more emphasis on the most neoplastic regions (i.e. those emphasized in the Hard-spot GT) because these are consistently present in all consensus GT masks. This approach enhances the model's ability to capture the subtle gradations of neoplasia, allowing it to delineate the extent of atypical tissue while identifying the most abnormal regions with increased intensity, \hlnew{which is in line with findings of our previous work~\citep{Kusters-CaPTion-GTConsensus}}. However, the quantitative performance is slightly lower compared to the Soft-spot GT and Plausible-spot GT training strategies.

These observations clearly indicate that the choice of segmentation GT has a substantial impact on the classification and localization performance. Incorporating gradations into segmentation GT allows the model to more effectively learn and capture the nuanced characteristics of neoplasia. Given these findings, the Plausible-spot GT training strategy is selected for the design of the CADe system due to its performance on low-quality imagery, which is often encountered in real-world settings. For better informed decision-making, the Multiple GT strategy might be considered instead. This approach improves the ability to differentiate between atypical tissue and the most abnormal regions, which is crucial for targeted biopsies, without significantly compromising overall performance.

% The classification, classification-by-segmentation and localization performance results of the optimal network architecture using previously selected training design choices with considered segmentation ground-truth utilization on the three validation sets are displayed in Table~\ref{table: ResultsDiscussion-Training-GT}. Furthermore, example lesions with corresponding Average GT and predicted segmentation masks of all the considered models are depicted in Fig.~\ref{fig: ResultsDiscussion-Training-GT}.

% For the performance on the Images+HQ Frames validation set, the model trained with Soft spot GT achieves the best performance with margins of 0.1\%, 0.1\% and 1.7\% for for AUROC$_{cls}$, AUPRC$_{cls}$ and $mD_i$, respectively. For AUROC$_{seg}$, the top performance is shared among the Soft spot, Plausible spot and Multiple GT strategies. Similarly, for AUPRC$_{seg}$, the highest scores are achieved by Soft spot, Plausible spot, Multiple and Average GT strategies. On the MQ Frames validation set, the model trained with Plausible spot GT achieves the best performance for all metrics with a consistent margin of 0.2\%. This trend continues on the LQ Frames validation set, where the Plausible spot GT strategy again secured the top performance, with margins of 0.2\%, 0.1\%, 0.5\% and 0.8\% for AUROC$_{cls}$, AUPRC$_{cls}$, AUROC$_{seg}$ and AUPRC$_{seg}$, respectively.

% The results clearly demonstrate a decline in performance, when transitioning from the model trained with Soft spot GT to the counterpart trained with Hard spot GT strategy. This decline is particularly pronounced in localization performance, as measured by $mD_i$, which shows a significant drop. This reduction in performance is due to the evaluation process relying on the default Plausible spot GT, which does not align with the smaller, more focused Hard spot GT strategy used during training. Furthermore, as illustrated in columns 3-6 of Fig.~\ref{fig: ResultsDiscussion-Training-GT}, there is a clear decrease in the size of the predicted segmentation masks, as the strategy shifts from Soft spot GT to Hard spot GT. This pattern reflects the differences in the training data, where the segmentation GT masks used in training vary in size and neoplastic certainty, as also illustrated in Fig.~\ref{fig: MaterialsMethods-Data-GroundTruth}. The Soft spot GT training strategy leads to large predicted masks with high confidence, capturing atypical and neoplastic areas with equal intensity. In contrast, the Hard spot GT training strategy results in highly condensed masks that focus intensively on the regions deemed most neoplastic during training. These findings suggest that training with masks that prioritize higher neoplastic certainty may inadvertently lead to the omission of subtle lesions, or subtle parts of larger lesions, thereby producing smaller predicted masks and ultimately deteriorating the detection performance. 

% Further interesting patterns emerge in columns 7-9 of Fig.~\ref{fig: ResultsDiscussion-Training-GT}. By the nature of the Random GT training strategy the model is forced to learn a generalized form of all consensus GT masks, which is evident in the predicted masks, as they are an intermediate form of the predicted masks of the Plausible spot GT and Sweet spot GT trained models. Both the Multiple GT and Average GT strategies expose the model to all consensus GT masks during training, but they lead to different outcomes. The Average GT approach results in segmentation masks with lower confidence, likely due to the non-binary nature causing predictions to be non-binary. In contrast, the Multiple GT strategy compels the model to generalize across all consensus GT masks, but with more emphasis on the most neoplastic regions (i.e. those emphasized in the Hard spot GT), as these are consistently present in all consensus GT masks. This approach enhances the model's ability to capture the subtle gradations of neoplasia, allowing it to delineate the extent of atypical tissue while identifying the most abnormal regions with increased intensity, which is in line with findings of previous work \textcolor{red}{\textbf{MICCAI}}. However, the quantitative performance is slightly lower compared to the Soft spot GT and Plausible spot GT training strategies. 

% These observations clearly indicate that the choice of segmentation GT has a substantial impact on the model's classification and localization performance. Incorporating gradations into segmentation GT allows the model to more effectively learn and capture the nuanced characteristics of neoplasia. Given these findings, the Plausible spot GT training strategy is selected for the design of the CADe system due to its performance on lower-quality imagery, which is often encountered in real-world settings. For the sake of better informed decision-making, the Multiple GT training strategy might be considered. This approach improves the model's ability to differentiate between atypical tissue and the most abnormal regions, which is crucial for targeted biopsies, without significantly compromising overall performance. 

%
\begin{table*}[t!]
    \centering
        \caption{Classification, classification-by-segmentation and localization performance of the optimal network architecture using previously selected training design choices with considered segmentation ground-truth utilization, on the different validation sets. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}
        \begin{tabular}{ l | c c c c c c c}
             \toprule
              \textbf{GT strategy} &\multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{cls}$ & AUPRC$_{cls}$ & $mD_i$ & AUROC$_{cls}$ & AUPRC$_{cls}$ & AUROC$_{cls}$ & AUPRC$_{cls}$ \\
             \midrule
             Soft-spot GT        & \textbf{0.972\sd{.002}} & \textbf{0.972\sd{.002}} & \textbf{0.636\sd{.020}} & 0.961\sd{.005} & 0.967\sd{.003} & 0.873\sd{.018} & 0.876\sd{.012}\\
             Plausible-spot GT   & 0.971\sd{.005} & 0.971\sd{.002} & 0.619\sd{.009} & \textbf{0.963\sd{.002}} & \textbf{0.969\sd{.001}} & \textbf{0.893\sd{.010}} & \textbf{0.888\sd{.011}}\\
             Sweet-spot GT       & 0.968\sd{.009} & 0.968\sd{.010} & 0.556\sd{.015} & 0.957\sd{.011} & 0.965\sd{.008} & 0.886\sd{.023} & 0.883\sd{.017}\\
             Hard-spot GT        & 0.964\sd{.009} & 0.961\sd{.012} & 0.379\sd{.012} & 0.953\sd{.004} & 0.960\sd{.004} & 0.870\sd{.012} & 0.867\sd{.013}\\
             Random GT           & 0.971\sd{.005} & 0.971\sd{.005} & 0.568\sd{.023} & 0.960\sd{.003} & 0.967\sd{.003} & 0.891\sd{.020} & 0.887\sd{.019}\\
             Multiple GT         & 0.970\sd{.003} & 0.968\sd{.006} & 0.593\sd{.022} & 0.957\sd{.003} & 0.965\sd{.003} & 0.882\sd{.018} & 0.880\sd{.018}\\
             Average FT          & 0.969\sd{.003} & 0.969\sd{.004} & 0.460\sd{.025} & 0.959\sd{.007} & 0.966\sd{.005} & 0.891\sd{.025} & 0.885\sd{.022}\\
            \midrule
            \midrule
             \textbf{GT strategy} & \multicolumn{3}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-6}
             \cmidrule(lr){7-8}
             & AUROC$_{seg}$ & AUPRC$_{seg}$ & & AUROC$_{seg}$ & AUPRC$_{seg}$ & AUROC$_{seg}$ & AUPRC$_{seg}$ \\
             \midrule
             Soft-spot GT        & \textbf{0.974\sd{.002}} & \textbf{0.973\sd{.002}} &  & 0.964\sd{.005} & 0.966\sd{.003} & 0.871\sd{.015} & 0.871\sd{.013}\\
             Plausible-spot GT  & \textbf{0.974\sd{.002}} & \textbf{0.973\sd{.003}} &  & \textbf{0.966\sd{.003}} & \textbf{0.968\sd{.002}} & \textbf{0.890\sd{.015}} & \textbf{0.882\sd{.012}}\\
             Sweet-spot GT      & 0.973\sd{.002} & 0.972\sd{.001} &  & 0.959\sd{.007} & 0.963\sd{.005} & 0.879\sd{.015} & 0.869\sd{.016}\\
             Hard-spot GT       & 0.968\sd{.006} & 0.967\sd{.005} &  & 0.953\sd{.003} & 0.960\sd{.001} & 0.869\sd{.005} & 0.856\sd{.006}\\
             Random GT          & 0.973\sd{.001} & 0.972\sd{.002} &  & 0.960\sd{.003} & 0.963\sd{.003} & 0.883\sd{.023} & 0.869\sd{.021}\\
             Multiple GT        & \textbf{0.974\sd{.003}} & \textbf{0.973\sd{.003}} &  & 0.961\sd{.004} & 0.965\sd{.004} & 0.885\sd{.014} & 0.874\sd{.011}\\
             Average GT          & 0.972\sd{.005} & \textbf{0.973\sd{.003}} &  & 0.961\sd{.005} & 0.966\sd{.003} & 0.884\sd{.014} & 0.874\sd{.014}\\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-Training-GT}
\end{table*}
%

%
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/GT Strategy/GroundTruthV2-cropped.pdf}
    \caption{Example lesions with corresponding Average GT and model predictions. In each row, the first column displays the original image, followed by the second column showing the corresponding Average GT mask. Subsequent columns present model predictions for training configurations using Soft-spot GT, Plausible-spot GT, Sweet-spot GT, Hard-spot GT, Random GT, Multiple GT, and Average GT, respectively. }
    \label{fig: ResultsDiscussion-Training-GT}
\end{figure*}
%



  % \begin{itemize}
  %   \item Domain-specific pre-training using an SSL objective enhances both model performance and robustness.
  %   \item Domain-specific data augmentation improves robustness but may negatively affect performance on clean, high-quality data.
  %   \item Incorporating lower-quality video frames in training enhances robustness, but results in a slight decrease in performance on clean data.
  %   \item The choice of multi-expert consensus GT significantly influences model performance. In any case, incorporating gradations within the GT enables more effective learning of subtle neoplastic characteristics.
  % \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: Inference strategies %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Inference strategies}
\label{sec: ResultsDiscussion-Inference}
This subsection presents and discusses the outcomes of the experiments conducted to evaluate the design choices regarding inference strategies, such as usage of model output and TensorRT inference, in Section~\ref{sec: ResultsDiscussion-Inference-OutputUsage} and \ref{sec: ResultsDiscussion-Inference-TensorRT}, respectively. 


\subsubsection{Usage of the model output - evaluation}
\label{sec: ResultsDiscussion-Inference-OutputUsage}
The classification performance of the optimal network architecture using previously selected training design choices with considered usage strategies of the model output, on the three validation sets are displayed in Table~\ref{table: ResultsDiscussion-Inference-OutputUsage}. The results indicate that deriving a single classification decision by combining the two outputs yields comparable or slightly improved performance compared to using either output individually. Particularly, both the average combination and the OR configuration outperform the best results of the individual outputs. The AND configuration can be considered too conservative by favoring the negative samples, while the OR configuration may be favoring the positive samples. The preferable performance of the average combination can be attributed to its utilization of both outputs for every sample, whereas the OR and AND configurations rely on a single output for AUROC and AUPRC computations. During training, each branch is supervised with either a classification label or a segmentation mask (not every training sample is paired with a segmentation mask). By integrating the two outputs, the strengths of both branches are combined, allowing outliers from one output to be counterbalanced by the other, thus providing a more consistent output. This effect is particularly pronounced in the LQ Frames validation set, where the lower image quality increases the likelihood of outlier predictions. As a result, the average combination strategy effectively neutralizes these outliers, leading to the highest performance improvements in this challenging scenario. These findings indicate that averaging the outputs of two branches is a robust strategy across different validation sets, especially in 'varying image quality' scenarios. Therefore, averaging the output of the classification branch and the maximum pixel value in the segmentation prediction is used as the strategy for the inference design of the CADe system in order to introduce more consistency in predictions.

% The classification performance of the optimal network architecture using previously selected training design choices with considered model output usage strategies on the three validation sets are displayed in Table~\ref{table: ResultsDiscussion-Inference-OutputUsage}. For the Images+HQ Frames validation set, the strategy of averaging the outputs from the classification and segmentation branches yielded the highest performance, outperforming other approaches by margins of 0.2\% for both AUROC and AUPRC. This trend is consistent across the MQ Frames validation set, where the average output strategy again achieved the best results, with improvements of 0.2\% and 0.3\% for AUROC and AUPRC, respectively. Similarly, on the LQ Frames validation set, this approach demonstrated the best performance, with even more pronounced margins of 0.6\% for AUROC and 0.4\% for AUPRC. 
% The results indicate that deriving a single classification decision by combining the two outputs yields comparable or slightly improved performance compared to using either output individually. Particularly, both the average combination and the OR configuration outperform the best results of the individual outputs. The AND configuration can be considered too conservative by favoring the negative samples, while the OR configuration may be favoring the positive samples. The preferable performance of the average combination can be attributed to its utilization of both outputs for every sample, whereas the OR and AND configurations rely on a single output for AUROC and AUPRC computations. During training, each branch is supervised with either a classification label or a segmentation mask, however, not every training sample is paired with a segmentation mask. By integrating the two outputs, the strengths of both branches are combined, allowing outliers from one output to be counterbalanced by the other, thus providing a more consistent output. This effect is particularly pronounced in the LQ Frames validation set, where the lower image quality increases the likelihood of outlier predictions. As a result, the average combination strategy effectively neutralizes these outliers, leading to the highest performance improvements in this challenging scenario. These findings indicate that averaging the outputs of two branches is a robust strategy across different validation sets, especially in varying image quality scenarios. Therefore, averaging the output of the classification branch and the maximum pixel value in the segmentation prediction is used as a strategy for the inference design of the CADe system in order to introduce more consistency in predictions. 

%
\begin{table*}[t!]
    \centering
        \caption{Classification performance of the optimal network architecture using previously selected training design choices with various usage strategies for inference model output, on the different validation sets. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}

        \begin{tabular}{ l | c c c c c c}
             \toprule
             \textbf{Model output} &\multicolumn{2}{ c }{\textbf{Images + HQ Frames}} & \multicolumn{2}{ c }{\textbf{MQ Frames}} & \multicolumn{2}{ c }{\textbf{LQ Frames}} \\
             \cmidrule{2-3}
             \cmidrule(lr){4-5}
             \cmidrule(lr){6-7}
             & AUROC & AUPRC & AUROC & AUPRC & AUROC & AUPRC \\
             \midrule
             Classification   & 0.971\sd{.005} & 0.971\sd{.004} & 0.963\sd{.002} & 0.969\sd{.001} & 0.893\sd{.010} & 0.888\sd{.011}\\
             Segmentation     & 0.974\sd{.002} & 0.973\sd{.003} & 0.966\sd{.003} & 0.968\sd{.002} & 0.890\sd{.015} & 0.882\sd{.012}\\
             Average          & \textbf{0.977\sd{.002}} & \textbf{0.975\sd{.003}} & \textbf{0.968\sd{.002}} & \textbf{0.972\sd{.002}} & \textbf{0.899\sd{.016}} & \textbf{0.892\sd{.014}}\\
             OR               & 0.975\sd{.002} & 0.973\sd{.003} & 0.966\sd{.003} & 0.969\sd{.002} & 0.893\sd{.017} & 0.885\sd{.013}\\
             AND              & 0.971\sd{.005} & 0.972\sd{.004} & 0.963\sd{.002} & 0.969\sd{.001} & 0.893\sd{.010} & 0.888\sd{.011}\\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-Inference-OutputUsage}
\end{table*}
%


\subsubsection{TensorRT inference - evaluation}
\label{sec: ResultsDiscussion-Inference-TensorRT}
The results demonstrate that TensorRT conversion can significantly enhance inference efficiency without compromising model performance, which also aligns with the findings of Zhou~\textit{et al.}~\citep{ZhouTensorRT}. Specifically, the average inference speed, measured over 5~repetitions of 1,000~samples each (with a 100-sample warm-up), increases by a factor of approximately~3.43, from 109.7~frames per second (fps) to 376.5~fps, when tested on a 40-GB A100 GPU (NVIDIA Corp., CA, USA). Importantly, the performance across the three validation sets remains unchanged. These results suggest that TensorRT conversion can offer substantial efficiency gains while preserving model effectiveness. This efficiency gain is particularly crucial for real-time applications, especially given the often slow pre/post-processing steps for input and output data. These steps, which were not accounted for in the current measurements, can significantly slow down overall inference time, making the observed improvements even more valuable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBSECTION: SOTA comparison %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{State-of-the-art comparison - evaluation}
\label{sec: ResultsDiscussion-SOTA}
Table~\ref{table: ResultsDiscussion-SOTA} presents a detailed comparison of the classification and localization performance or the proposed model against several state-of-the-art CADe systems for Barrett's neoplasia detection. This comparison spans various test sets, focusing on peak performance, generalization and robustness. The results show that the proposed CADe system significantly outperforms existing state-of-the-art models in terms of both AUROC and AUPRC across all tests sets ($p=0.0019$). For localization performance, measured by $mD_i$, the proposed model also demonstrates superior performance, achieving statistical significance across all models ($p=0.018$) and slightly less significant for the model of De~Groof~\textit{et al.}~\citep{DeGroof} ($p=0.031$). In the following subsections, the results on peak performance, generalization and robustness are highlighted separately. The results demonstrate that the proposed model is well-equipped for practical applications, with significant improvements over state-of-the-art CADe models, especially for endoscopy-specific, clinically relevant robustness.

% All sets AUROC: 0.001953, AUPRC: 0.001953, mDi: 0.01875 (De Groof 0.03125)

\begin{table*}[t!]
    \centering
        \caption{Classification and localization performance comparison of the optimal network architecture using previously selected training and inference design choices against state-of-the-art architectures, on the different test sets. The table is partitioned in four sections, each with one specific performance objective. The third section has generalization at the left and robustness at the right as an objective. Results are presented as Mean $\pm$ Std. The best results are highlighted in boldface.}
        \begin{tabular}{ l | c c c c c c}
             \toprule
              \textbf{SOTA comparison} &\multicolumn{3}{ c }{\textbf{BM Test}} & \multicolumn{3}{ c }{\textbf{AC Test}} \\
             \cmidrule{2-4}
             \cmidrule(lr){5-7}
             \textcolor{gray}{\textit{Peak performance}} & AUROC & AUPRC & $mD_i$ & AUROC & AUPRC & $mD_i$\\
             \midrule
             Ebigbo \textit{et al.}~\citep{Ebigbo}          & 0.930\sd{.014} & 0.873\sd{.022} & 0.497\sd{.026} & 0.962\sd{.005} & 0.897\sd{.019} & 0.607\sd{.014} \\
             de Groof \textit{et al.}~\citep{DeGroof}       & 0.927\sd{.015} & 0.869\sd{.024} & 0.493\sd{.035} & 0.944\sd{.011} & 0.890\sd{.021} & 0.652\sd{.026} \\
             Hussein \textit{et al.}~\citep{Hussein}        & 0.946\sd{.011} & 0.900\sd{.017} & 0.498\sd{.036} & 0.965\sd{.011} & 0.921\sd{.019} & 0.624\sd{.019} \\
             Abdelrahim \textit{et al.}~\citep{Abdelrahim}  & 0.919\sd{.012} & 0.862\sd{.015} & 0.437\sd{.075} & 0.942\sd{.012} & 0.874\sd{.030} & 0.580\sd{.036} \\
             Fockens \textit{et al.}~\citep{FockensBE2}     & 0.954\sd{.010} & 0.912\sd{.013} & 0.463\sd{.015} & 0.966\sd{.008} & 0.923\sd{.008} & 0.533\sd{.004} \\
             Meinikheim \textit{et al.}~\citep{Meinikheim}  & 0.938\sd{.007} & 0.891\sd{.011} & 0.469\sd{.036} & 0.951\sd{.008} & 0.900\sd{.006} & 0.607\sd{.009} \\
             \midrule
             Proposed                                           & \textbf{0.977\sd{.002}} & \textbf{0.952\sd{.004}} & \textbf{0.587\sd{.015}} & \textbf{0.990\sd{.002}} & \textbf{0.968\sd{.005}} & \textbf{0.663\sd{.011}} \\
            \midrule
            \midrule
             \textbf{SOTA comparison} & \multicolumn{3}{ c }{\textbf{ARGOS DS 3+4}} & \multicolumn{3}{ c }{\textbf{ARGOS DS 5}}\\
             \cmidrule{2-4}
             \cmidrule(lr){5-7}
             \textcolor{gray}{\textit{Generalization}} & AUROC & AUPRC & $mD_i$ & AUROC & AUPRC & $mD_i$\\
             \midrule
             Ebigbo \textit{et al.}~\citep{Ebigbo}          & 0.936\sd{.005} & 0.932\sd{.009} & 0.618\sd{.009} & 0.933\sd{.011} & 0.932\sd{.020} & 0.595\sd{.027}\\
             de Groof \textit{et al.}~\citep{DeGroof}       & 0.941\sd{.008} & 0.936\sd{.008} & 0.620\sd{.034} & 0.938\sd{.016} & 0.944\sd{.018} & \textbf{0.619\sd{.054}}\\
             Hussein \textit{et al.}~\citep{Hussein}        & 0.938\sd{.010} & 0.933\sd{.012} & 0.631\sd{.006} & 0.939\sd{.006} & 0.949\sd{.007} & 0.604\sd{.010}\\
             Abdelrahim \textit{et al.}~\citep{Abdelrahim}  & 0.924\sd{.009} & 0.915\sd{.015} & 0.569\sd{.048} & 0.925\sd{.018} & 0.926\sd{.031} & 0.541\sd{.052}\\
             Fockens \textit{et al.}~\citep{FockensBE2}     & 0.939\sd{.005} & 0.939\sd{.008} & 0.482\sd{.010} & 0.932\sd{.007} & 0.942\sd{.009} & 0.454\sd{.021}\\
             Meinikheim \textit{et al.}~\citep{Meinikheim}  & 0.951\sd{.003} & 0.949\sd{.005} & 0.632\sd{.009} & 0.914\sd{.009} & 0.920\sd{.015} & 0.590\sd{.020}\\
             \midrule
             Proposed                                           & \textbf{0.975\sd{.004}} & \textbf{0.974\sd{.002}} & \textbf{0.644\sd{.010}} & \textbf{0.963\sd{.006}} & \textbf{0.971\sd{.004}} & 0.609\sd{.015}\\
                 \midrule
            \midrule
             \textbf{SOTA comparison} & \multicolumn{3}{ c }{\textbf{BORN}} & \multicolumn{3}{ c }{\textbf{BM Test-C}}\\
             \cmidrule{2-4}
             \cmidrule(lr){5-7}
             \textcolor{gray}{\textit{Generalization \& Robustness}} & AUROC & AUPRC & $mD_i$ & AUROC & AUPRC & $mD_i$\\
             \midrule
             Ebigbo \textit{et al.}~\citep{Ebigbo}          & 0.900\sd{.011} & 0.867\sd{.012} & 0.405\sd{.010} & 0.821\sd{.020} & 0.712\sd{.040} & 0.285\sd{.026} \\
             de Groof \textit{et al.}~\citep{DeGroof}       & 0.896\sd{.020} & 0.863\sd{.023} & 0.398\sd{.027} & 0.815\sd{.021} & 0.715\sd{.030} & 0.297\sd{.025} \\
             Hussein \textit{et al.}~\citep{Hussein}        & 0.890\sd{.011} & 0.859\sd{.016} & 0.410\sd{.037} & 0.826\sd{.010} & 0.739\sd{.014} & 0.287\sd{.017} \\
             Abdelrahim \textit{et al.}~\citep{Abdelrahim}  & 0.910\sd{.016} & 0.878\sd{.024} & 0.407\sd{.040} & 0.825\sd{.033} & 0.717\sd{.043} & 0.289\sd{.079} \\
             Fockens \textit{et al.}~\citep{FockensBE2}     & 0.895\sd{.011} & 0.869\sd{.013} & 0.339\sd{.014} & 0.853\sd{.010} & 0.760\sd{.014} & 0.295\sd{.007}\\
             Meinikheim \textit{et al.}~\citep{Meinikheim}  & 0.878\sd{.005} & 0.842\sd{.007} & 0.372\sd{.023} & 0.824\sd{.016} & 0.722\sd{.026} & 0.276\sd{.030} \\
             \midrule
             Proposed                                           & \textbf{0.915\sd{.006}} & \textbf{0.884\sd{.008}} & \textbf{0.472\sd{.019}} & \textbf{0.915\sd{.008}} & \textbf{0.874\sd{.009}} & \textbf{0.425\sd{.012}} \\
             \midrule
             \midrule
            \textbf{SOTA comparison} & \multicolumn{2}{ c }{\textbf{IQ Triplet - HQ}} & \multicolumn{2}{ c }{\textbf{IQ Triplet - MQ}} & \multicolumn{2}{ c }{\textbf{IQ Triplet - LQ}}\\
             \cmidrule{2-4}
             \cmidrule(lr){2-3}
             \cmidrule(lr){4-5}
             \cmidrule(lr){6-7}
             \textcolor{gray}{\textit{Robustness}} & AUROC & AUPRC & AUROC & AUPRC & AUROC & AUPRC  \\
             \midrule
             Ebigbo \textit{et al.}~\citep{Ebigbo}          & 0.970\sd{.007} & 0.976\sd{.005} & 0.939\sd{.011} & 0.948\sd{.011} & 0.794\sd{.016} & 0.841\sd{.016} \\
             de Groof \textit{et al.}~\citep{DeGroof}       & 0.963\sd{.011} & 0.972\sd{.008} & 0.913\sd{.015} & 0.937\sd{.012} & 0.816\sd{.012} & 0.853\sd{.022} \\
             Hussein \textit{et al.}~\citep{Hussein}        & 0.978\sd{.010} & 0.983\sd{.007} & 0.937\sd{.008} & 0.955\sd{.008} & 0.803\sd{.024} & 0.851\sd{.017} \\
             Abdelrahim \textit{et al.}~\citep{Abdelrahim}  & 0.969\sd{.011} & 0.978\sd{.008} & 0.914\sd{.019} & 0.941\sd{.015} & 0.762\sd{.022} & 0.806\sd{.013} \\
             Fockens \textit{et al.}~\citep{FockensBE2}     & 0.979\sd{.005} & 0.985\sd{.004} & 0.926\sd{.021} & 0.947\sd{.014} & 0.829\sd{.021} & 0.869\sd{.026} \\
             Meinikheim \textit{et al.}~\citep{Meinikheim}  & 0.970\sd{.005} & 0.978\sd{.003} & 0.949\sd{.006} & 0.964\sd{.004} & 0.829\sd{.020} & 0.856\sd{.017} \\
             \midrule
             Proposed                                           & \textbf{0.994\sd{.003}} & \textbf{0.994\sd{.003}} & \textbf{0.976\sd{.005}} & \textbf{0.978\sd{.005}} & \textbf{0.911\sd{.014}} & \textbf{0.929\sd{.009}} \\
             \bottomrule
        \end{tabular}
    \label{table: ResultsDiscussion-SOTA}
\end{table*}
%

\subsubsection{Peak performance}
For the BM Test set, which is intentionally enriched with subtle neoplastic cases that pose significant challenges for endoscopists in clinical practice, the proposed model demonstrates superior performance across all evaluation metrics, with improvements up to 8.9\%. Similarly, on the AC Test set, which comprises consecutive cases recorded over a two-month period and represents the full spectrum of scenarios encountered in routine clinical practice, the proposed model again outperforms its counterparts with margins up to 4.5\%. Overall, across all metrics for the peak performance test sets, the proposed model achieves statistically significant improvements over state-of-the-art CADe models ($p=0.015$). These results underscore the superiority of the proposed model, particularly in handling both highly challenging and real-world clinical cases, which demonstrates its potential for practical and clinical applications.

% For the BM Test set, which is intentionally enriched with subtle neoplastic cases that pose significant challenges for endoscopists in clinical practice, the proposed model demonstrates superior performance across all evaluation metrics. Specifically, it achieves margins of 2.3\%, 4\% and 8.9\% for AUROC, AUPRC and $mD_i$, respectively. Similarly, on the AC Test set, which comprises consecutive cases recorded over a two-month period and represents the full spectrum of scenarios encountered in routine clinical practice, the proposed model again outperforms its counterparts with margins of 2.4\%, 4.5\% and 1.1\% for AUROC, AUPRC and $mD_i$, respectively. Overall, across all metrics for the peak performance test sets, the proposed model achieves statistically significant improvements over state-of-the-art CADe models ($p=0.015$). These results underscore the superiority of our model, particularly in handling both highly challenging and real-world clinical cases, demonstrating potential for practical applications.

% Peak performance - All metrics: 0.015625

\subsubsection{Generalization}
For the ARGOS DS 3+4 test set, which is a heterogeneous dataset characterized by varying lesion subtlety and captured with gastroscopes from a different manufacturer than those used for the development data, the proposed model consistently outperforms all other models across all evaluation metrics. Specifically, it achieves improvements up to 2.5\%. Similarly, on the ARGOS DS 5 test set, which is artificially enriched with subtle neoplastic lesions and also recorded with gastroscopes from another manufacturer, the proposed model again shows superior classification performance with margins up to 2.7\%. However, in terms of localization performance, the model by De~Groof~\textit{et al.}~\citep{DeGroof} outperforms the proposed model by 1\%. For the BORN test set, which was acquired using older generation gastroscopes and other manufacturer's devices, leading to data with lower objective quality compared to the development data, the proposed model achieves a substantial 6.2\% margin for localization performance, while classification performance is comparable. Across all metrics for the generalization performance test sets, the proposed model consistently achieves statistically significant improvements over state-of-the-art CADe models ($p=0.0023$). Even when compared to the model of De~Groof~\textit{et al.}, which performs slightly better in a single metric, the proposed model maintains significant advantages ($p=0.0039$). These findings highlight the superior generalization capabilities of the proposed model, particularly in handling variations in objective image quality and adapting to diverse data sources, including older generation scopes and devices from different manufacturers.

% For the ARGOS DS 3+4 test set, which is a heterogeneous dataset characterized by varying lesion subtlety and captured using gastroscopes from a different manufacturer than those used for the development data, the proposed model consistently outperforms all other models across all evaluation metrics. Specifically, it achieves improvements of 2.4\% in AUROC, 2.5\% in AUPRC, and 1.2\% in $mD_i$. Similarly, on the ARGOS DS 5 test set, which is artificially enriched with subtle neoplastic lesions and also recorded with gastroscopes from another manufacturer, the proposed model again shows superior performance in AUROC and AUPRC, with respective margins of 2.4\% and 2.7\%. However, in terms of localization performance as measured by $mD_i$, the model by De Groof~\textit{et al.}~\citep{DeGroof} outperforms our model by 1\%. For the BORN test set, which was acquired using older generation gastroscopes and other manufacturer's devices, leading to data with lower objective quality compared to the development data, the proposed model achieves margins of 0.5\% in AUROC, 0.6\% in AUPRC and a substantial 6.2\% in $mD_i$. Across all metrics for the generalization performance test sets, the proposed model consistently achieves statistically significant improvements over state-of-the-art CADe models ($p=0.0023$). Even when compared to the model of De Groof~\textit{et al.}, which performs slightly better in a single metric, the proposed model maintains significant advantages ($p=0.0039$). These findings highlight the superior generalization capabilities of our model, particularly in handling variations in objective image quality and adapting to diverse data sources, including older generation scopes and devices from different manufacturers.  

% Generalization - All metrics: 0.002344 (De Groof 0.003906)

\subsubsection{Robustness}
For the BM Test-C set, which includes the BM Test data with clinically realistic and endoscopy-specific calibrated synthesized corruptions, the proposed model achieves significant margins up to 12.8\% on the performance metrics. In the IQ Triplet test sets, comprising three subsets with matched triplets across distinct levels of image quality, the proposed model shows consistent improvements over the state-of-the-art CADe models. For the HQ subset, the model achieves a maximal gain of 1.5\%, while the MQ subset reveals even greater margins of up to 2.7\%. The most pronounced gains are observed in the LQ subset, with a maximum margin of 8.2\%. Across all metrics for the robustness test sets, the proposed model consistently demonstrates statistically significant improvements over state-of-the-art CADe models ($p=0.0019$). These findings underscore the superior robustness of the proposed model, particularly in managing endoscopy-specific artificial corruptions and real-world low-quality data.

% For the BM Test-C set, which includes the BM Test data with clinically realistic and endoscopy-specific calibrated synthesized corruptions, the proposed model achieves significant margins of 6.2\%, 11.4\% and 12.8\% for AUROC, AUPRC, and $mD_i$, respectively. In the IQ Triplet test sets, comprising three subsets with matched triplets across distinct levels of image quality, the proposed model shows consistent improvements over the state-of-the-art CADe models. For the HQ subset, the model achieves gains of 1.5\% in AUROC and 0.9\% in AUPRC. The MQ subset reveals even greater margins, with improvements of 2.7\% and 1.4\% for AUROC and AUPRC, respectively. The most pronounced gains are observed in the LQ subset, with margins of 8.2\% and 6\% for AUROC and AUPRC, respectively. Across all metrics for the robustness test sets, the proposed model consistently demonstrates statistically significant improvements over state-of-the-art CADe models ($p=0.0019$). These findings underscore the superior robustness of our model, particularly in managing endscopy-specific artificial corruptions and real-world lower-quality data.

% Robustness - All metrics: 0.001953


\begin{tcolorbox}[colback=white,colframe=black!75!white,title=Key findings: Training strategies]
  \begin{itemize}[noitemsep]
    \item Domain-specific pre-training using an SSL objective enhances both model performance and robustness.
    \item Domain-specific data augmentation improves robustness but may negatively affect performance on clean, high-quality data.
    \item Incorporating lower-quality video frames in training enhances robustness, but results in a slight decrease in performance on clean data.
    \item The choice of multi-expert consensus GT significantly influences model performance. In any case, incorporating gradations within the GT enables more effective learning of subtle neoplastic characteristics.
  \end{itemize}
\end{tcolorbox}

\begin{tcolorbox}[colback=white,colframe=black!75!white,title=Key findings: Inference approaches]
  \begin{itemize}[noitemsep]
    \item Combining the classification and segmentation branch outputs leads to improved classification performance and greater consistency compared to using a single output.
    \item TensorRT conversion delivers significant efficiency improvements without compromising model effectiveness.
  \end{itemize}
\end{tcolorbox}

==> Sections/6-Conclusions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONCLUSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Motivation}
\textsc{A. Motivation}: Early detection of neoplastic lesions in Barrett's Esophagus (BE) is challenging due to the subtle endoscopic appearance and the potential biopsy sampling errors, highlighting the need for advanced Computer-Aided Detection (CADe) systems to assist endoscopists in accurately identifying and localizing neoplasia. The development of such systems hinges on several key design decisions, particularly the selection of the network architecture. Whereas Convolutional Neural Networks (CNNs) have traditionally dominated this space, recent innovations such as Vision Transformers (ViTs) and State-Space Models (SSMs) bring new opportunities to enhance CADe performance. Each of these architectures offers unique strengths and limitations that can significantly affect clinical outcomes. 
Variability in endoscopic image quality, originating from factors like motion blur, lighting conditions and device differences, pose a significant challenge for deep learning-based techniques. Effective CADe systems must not only excel in controlled environments, but also demonstrate robustness and generalization across a wide range of real-world clinical scenarios. Moreover, the success of these systems in clinical practice is heavily dependent on their consistency and localization accuracy, which directly impact endoscopist compliance. Therefore, in addition to architectural choices it is essential to explore and optimize various training and inference strategies that can enhance model performance, consistency and precise localization accuracy, ensuring the effectiveness of CADe systems in aiding the detection of neoplasia in BE.


% \subsection{Contributions}
\textsc{B. Contributions}: This paper has provided an in-depth evaluation of architectural choices, training strategies and inference approaches to offer valuable insights for the structured design and development of CADe systems for Barrett's neoplasia detection. The evaluation specifically addresses the unique challenges and complexities associated with endoscopic imaging and the nature of Barrett's neoplasia. The evaluation of architectures encompassed 10 backbone architectures and 4 semantic segmentation decoder architectures. Among the training strategies, domain-specific pre-training with an SSL objective, data augmentation techniques, training with additional video frames and utilization of multi-expert segmentation ground-truth are evaluated. For the inference strategies, several model output fusion techniques and TensorRT conversion are evaluated. The results demonstrate that the incorporation of structured design considerations leads to measurable and incremental performance improvements for all design objectives. The contributions particularly stand out for the domain-specific pre-training and the use of a hybrid CNN-Transformer architecture, which benefits robustness and overall performance. The resulting model with optimal design choices is benchmarked against 6 state-of-the-art CADe systems for Barrett's neoplasia detection, in terms of peak performance, generalization, and robustness, across 9 diverse tests tests reflecting real-world clinical challenges. The proposed model achieves statistically significant improvements over the existing CADe systems in both classification and localization.  


% \subsection{Limitations}
\textsc{C. Limitations}: The experimental design and analysis presented in this study, although thorough, introduce potential limitations that should be acknowledged. Firstly, a uniform training procedure is applied across all models to ensure experimental consistency, with variations limited only to the learning rate. This approach is employed for model backbone selection, decoder selection, and comparisons with state-of-the-art methods, except for the model of Fockens~\textit{et al.}~\citep{FockensBE2}. While this uniformity is considered as the most equitable for comparison, it may result in suboptimal hyperparameters for certain models and does not fully account for uncertainty inherently present in the hyperparameter space. Additionally, the experiments concerning design choices for training strategies are conducted in a sequential manner. The sequence of these design choices can influence the results. For instance, domain-specific pre-training is evaluated first, and leads to significant performance gains setting a performance baseline that makes subsequent improvements from other design choices appear marginal. Although this approach is logical given the significance of domain-specific pre-training, alternative sequences or independent evaluations of each strategy can potentially yield supplementary insights. Moreover, in the domain-specific pre-training experiments, only a single self-supervised learning objective has been considered. The final aim is not to provide insights in these SSL objectives per se, as this is described extensively in our previous work~\citep{BoersMEDIA}, but rather to demonstrate the clear benefits of in-domain pre-training using any SSL objective. Finally, the experiments involving additional video frames are limited by the availability of frames from a restricted patient pool. This limitation inherently reduces the diversity of the frames for training, which in turn constrains the potential performance gains. Ideally, this experiment should be repeated with a more diverse set of video frames sourced from a larger patient population to better assess generalization of the findings. 


==> Sections/7-Acknowledgments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACKNOWLEDGMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This work is facilitated by data and equipment from Olympus Corp., Tokyo, Japan. Therefore, we want to gratefully acknowledge Olympus for the provided research support. Furthermore, we thank SURF (\url{www.surf.nl}) for the support in using the National Supercomputer Snellius.
